Accuracy Can Lie: On the Impact of Surrogate Model in Configuration Tuning

To ease the expensive measurements during configuration tuning, it is natural to build a surrogate model as the replacement of the system, and thereby the configuration performance can be cheaply evaluated. Yet, a stereotype therein is that the higher the model accuracy, the better the tuning result would be. This "accuracy is all" belief drives our research community to build more and more accurate models and criticize a tuner for the inaccuracy of the model used. However, this practice raises some previously unaddressed questions, e.g., Do those somewhat small accuracy improvements reported in existing work really matter much to the tuners? What role does model accuracy play in the impact of tuning quality? To answer those related questions, we conduct one of the largest-scale empirical studies to date-running over the period of 13 months 24*7-that covers 10 models, 17 tuners, and 29 systems from the existing works while under four different commonly used metrics, leading to 13,612 cases of investigation. Surprisingly, our key findings reveal that the accuracy can lie: there are a considerable number of cases where higher accuracy actually leads to no improvement in the tuning outcomes (up to 58% cases under certain setting), or even worse, it can degrade the tuning quality (up to 24% cases under certain setting). We also discover that the chosen models in most proposed tuners are sub-optimal and that the required % of accuracy change to significantly improve tuning quality varies according to the range of model accuracy. Deriving from the fitness landscape analysis, we provide in-depth discussions of the rationale behind, offering several lessons learned as well as insights for future opportunities. Most importantly, this work poses a clear message to the community: we should take one step back from the natural "accuracy is all" belief for model-based configuration tuning.

==> Figures/RQ2/rq2_result.tex <==
\begin{figure}[t!]
\centering
\subfloat[The count result of SMBO match results]{%
  \begin{tikzpicture}
      \begin{axis}[
                ymajorgrids=true,
          ybar,
          bar width=.3cm,
          width=0.55\textwidth,
          height=.3\textwidth,
          legend image code/.code={%
                    \draw[#1] (0cm,-0.1cm) rectangle (0.1cm,0.15cm);
                }, 
          legend style={at={(0.5,1.25)},
              anchor=north,legend columns=-1,font=\tiny,nodes={scale=1, transform shape},draw=none,fill=none,},
          xtick=data,
          xticklabels={MAPE--PERF.,µRD--PERF., MAPE--EFF.,µRD--EFF.},
          nodes near coords = {\tiny\pgfmathprintnumber[fixed, precision=1]{\pgfplotspointmeta}},
          nodes near coords align={vertical},
          ymin=0, ymax=150,
          font=\tiny,
          ylabel={Count},
          ylabel style={yshift=-2em},
          % xlabel={Match},
          % ylabel style={yshift=-10pt}
          enlarge x limits={abs=0.8cm},  % 调整左右边界
          % extra y ticks={20,40,60,80,100},
          % extra y tick style={grid=major},
          grid style = {dashed},
          % grid=both
          ]
          % 柱状图
          \addplot[fill=blue!30] coordinates {(1, 29) (2, 30) (3, 15) (4, 23)};
          \addplot[fill=red!30] coordinates {(1, 24) (2, 32) (3, 31) (4, 21)};
          \addplot[fill=green!30] coordinates {(1, 53) (2, 62) (3, 46) (4, 44)};
          \legend{Best Match, Worst Match, All Match}
      \end{axis}
  \end{tikzpicture}%
  \label{fig:left_plot}%
}
\hfill
\subfloat[The count result of MFO match results]{%
  \begin{tikzpicture}
      \begin{axis}[
                ymajorgrids=true,
          ybar,
          bar width=.3cm,
          width=0.55\textwidth,
          height=.3\textwidth,
          legend image code/.code={%
                    \draw[#1] (0cm,-0.1cm) rectangle (0.1cm,0.15cm);
                }, 
          legend style={at={(0.5,1.25)},
              anchor=north,legend columns=-1,font=\tiny,nodes={scale=1, transform shape},draw=none,fill=none,},
          xtick=data,
          xticklabels={MAPE--PERF.,µRD--PERF., MAPE--EFF.,µRD--EFF.},
          nodes near coords = {\tiny\pgfmathprintnumber[fixed, precision=1]{\pgfplotspointmeta}},
          nodes near coords align={vertical},
          ymin=0, ymax=150,
          font=\tiny,
          ylabel={Count},
          ylabel style={yshift=-2em},
          % xlabel={Match},
          % ylabel style={yshift=-10pt}
          enlarge x limits={abs=0.8cm},  % 调整左右边界
          % extra y ticks={20,40,60,80,100},
          % extra y tick style={grid=major},
          grid style = {dashed},
          % grid=both
          ]
          % 柱状图
          \addplot[fill=blue!30] coordinates {(1, 63) (2, 58) (3, 23) (4, 28)};
          \addplot[fill=red!30] coordinates {(1, 44) (2, 64) (3, 37) (4, 49)};
          \addplot[fill=green!30] coordinates {(1, 107) (2, 122) (3, 60) (4, 77)};
          \legend{Best Match, Worst Match, All Match}
      \end{axis}
  \end{tikzpicture}%
  \label{fig:right_plot}%
}
\caption{The overall ratio of count of RQ2 results}
\label{fig:rq1_MFO_combined}
\end{figure}

==> Figures/RQ3/rq3_result.tex <==
\begin{figure*}[t!]
\centering
\subfloat[The count of SMBO Spearman correlation results]{%
  \begin{tikzpicture}
      \begin{axis}[
          ymajorgrids=true,
          % xmajorgrids=true,
          ybar,
          bar width=.25cm,
          width=\textwidth,
          height=.3\textwidth,
          legend image code/.code={%
                    \draw[#1] (0cm,-0.1cm) rectangle (0.15cm,0.15cm);
                }, 
          legend style={at={(0,1.2)},
              anchor=west,legend columns=5,font=\small,nodes={scale=1, transform shape},draw=none,fill=none,},
          xtick=data,
          xticklabels={PERF--MAPE.,PERF.--$\mu$RD, EFF.--MAPE,EFF.--$\mu$RD},
          nodes near coords = {\tiny\pgfmathprintnumber[fixed, precision=1]{\pgfplotspointmeta}},
          nodes near coords align={vertical},
          ymin=-5, ymax=150,
          font=\small,
          ylabel={\# cases},
          ylabel style={yshift=-1em},
          % xlabel={Match},
          % ylabel style={yshift=-10pt}
          enlarge x limits={abs=1.5cm},  % 调整左右边界
          % extra y ticks={20,40,60,80,100},
          % extra y tick style={grid=major},
          grid style = {dashed},
          % grid=both
          ]
          % 柱状图
          
          % the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.
          \addplot[fill=red!100] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          \addplot[fill=red!50] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          \addplot[fill=red!30] coordinates {(1, 8) (2, 0) (3, 4) (4, 5)};
          \addplot[fill=red!10] coordinates {(1, 24) (2, 18) (3, 54) (4, 28)};
          % \addplot[fill=red!10] coordinates {(1, 55) (2, 68) (3, 85) (4, 75)};
          \addplot[fill=gray!10] coordinates {(1, 105) (2, 84) (3, 111) (4, 136)};
          % \addplot[fill=blue!10] coordinates {(1, 55) (2, 68) (3, 85) (4, 75)};
          \addplot[fill=blue!10]  coordinates {(1, 67) (2, 87) (3, 60) (4, 55)};
          \addplot[fill=blue!30] coordinates {(1, 27) (2, 41) (3, 3) (4, 8)};
          \addplot[fill=blue!60] coordinates {(1, 1) (2, 2) (3, 0) (4, 0)};
          \addplot[fill=blue!100] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};

          
          \legend{Very strong negtive, Strong negtive, Moderate negtive, Weak negtive,
          Negligible, Weak postive, Moderate postive, Strong postive, Very strong postive,}
      \end{axis}
  \end{tikzpicture}%
  \label{fig:rq3_SMBO}%
}
\hfill
\subfloat[The count of MFO Spearman correlation results]{%
  \begin{tikzpicture}
      \begin{axis}[
          ymajorgrids=true,
          ybar,
          bar width=.25cm,
          width=\textwidth,
          height=.3\textwidth,
          legend style={at={(0,1.2)},
              anchor=west,legend columns=5,font=\small,nodes={scale=1, transform shape},draw=none,fill=none,},
          xtick=data,
          xticklabels={PERF--MAPE.,PERF.--$\mu$RD, EFF.--MAPE,EFF.--$\mu$RD},
          nodes near coords = {\tiny\pgfmathprintnumber[fixed, precision=1]{\pgfplotspointmeta}},
          nodes near coords align={vertical},
          ymin=-5, ymax=150,
          font=\small,
          ylabel={\# cases},
          ylabel style={yshift=-1em},
          % xlabel={Match},
          % ylabel style={yshift=-10pt}
          enlarge x limits={abs=1.5cm},  % 调整左右边界
          % extra y ticks={20,40,60,80,100},
          % extra y tick style={grid=major},
          grid style = {dashed},
          % grid=both
          ]
          % 柱状图
          % the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.
          \addplot[fill=red!100] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          \addplot[fill=red!50] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          \addplot[fill=red!30] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          \addplot[fill=red!10] coordinates {(1, 0) (2, 0) (3, 10) (4, 7)};
          % \addplot[fill=red!10] coordinates {(1, 55) (2, 68) (3, 85) (4, 75)};
          \addplot[fill=gray!10] coordinates {(1, 34) (2, 23) (3, 94) (4, 86)};
          % \addplot[fill=blue!10] coordinates {(1, 55) (2, 68) (3, 85) (4, 75)};
          \addplot[fill=blue!10]  coordinates {(1, 69) (2, 55) (3, 60) (4, 66)};
          \addplot[fill=blue!30] coordinates {(1, 62) (2, 77) (3, 8) (4, 13)};
          \addplot[fill=blue!60] coordinates {(1, 11) (2, 21) (3, 4) (4, 4)};
          \addplot[fill=blue!100] coordinates {(1, 0) (2, 0) (3, 0) (4, 0)};
          
      \end{axis}
  \end{tikzpicture}%
  \label{fig:rq3_MFO}%
}

\caption{The overall count of RQ3 results}
\label{fig:rq3_result}
\end{figure*}

==> Figures/RQ4/rq4_results.tex <==

\begin{figure}[t]
    \centering

    
    

    \pgfplotstableread[row sep=\\,col sep=&]{
        index & PERF.--MFO & EFF.--MFO & PERF.--SMBO & EFF.--SMBO \\
        10 & 0.81 & 0.89 & 0.84 & 0.76 \\
        20 & 8.76 & 9.55 & 5.30 & 5.32 \\
        30 & 12.38 & 12.91 & 7.65 & 8.39 \\
        40 & 20.45 & 21.13 & 14.76 & 12.50 \\
        50 & 32.39 & 28.48 & 24.81 & 23.53 \\
        60 & 26.16 & 28.97 & 25.17 & 20.42 \\
        70 & 42.45 & 42.64 & 26.44 & 23.61 \\
        80 & 55.88 & 58.23 & 29.43 & 37.17 \\
        90 & 59.51 & 65.07 & 32.85 & 34.83 \\
        100 & 66.23 & 105.62 & 73.18 & 60.47 \\
    }\mydata
    
    \begin{tikzpicture}
        \begin{axis}[
                grid style = {dashed},
                ymajorgrids=true,
                ybar,
                bar width=.15cm,
                width=0.92\textwidth,
                height=.5\textwidth,
                legend style={at={(0.5,0.99)},
                    anchor=north,legend columns=-1,font=\small},
                xtick=data,
                xticklabels={0--10,10--20,20--30,30--40,40--50,50--60,60--70,70--80,80--90,90--100},
                % nodes near coords={\tiny\pgfmathprintnumber{\pgfplotspointmeta}}, % 设置数据标签为小号字体,
                % 使用 \pgfplotspointmeta 来显示数据标签
                nodes near coords align={vertical},
                ymin=0,ymax=120,
                ylabel={Improvement (\%)},
                xlabel={Ranges (\%)},
                % extra y ticks={20,40,60,80,100},
                % extra y tick style={grid=major},
                enlarge x limits={abs=0.5cm},  % 调整左右边界
                % xtick style={draw=none}, % 去掉x轴刻度
                % tick align=inside, % 刻度超内
                ylabel style={yshift=-1em},
            ]
            % 柱状图
            \addplot[fill=blue!30] table[x=index,y=PERF.--MFO]{\mydata};
            \addplot[fill=red!30] table[x=index,y=EFF.--MFO]{\mydata};
            \addplot[fill=green!30] table[x=index,y=PERF.--SMBO]{\mydata};
            \addplot[fill=orange!30] table[x=index,y=EFF.--SMBO]{\mydata};

            % 折线图
            \addplot[smooth,mark=*,mark size=1pt,blue] table[x expr=\thisrow{index}-3.2,y=PERF.--MFO]{\mydata};
            \addplot[smooth,mark=*,mark size=1pt,red] table[x expr=\thisrow{index}-1.1,y=EFF.--MFO]{\mydata};
            \addplot[smooth,mark=*,mark size=1pt,green] table[x expr=\thisrow{index}+1.1,y=PERF.--SMBO]{\mydata};
            \addplot[smooth,mark=*,mark size=1pt,orange] table[x expr=\thisrow{index}+3.2,y=EFF.--SMBO]{\mydata};
            \legend{PERF.--MFO, EFF.--MFO, PERF.--SMBO, EFF.--SMBO}
        \end{axis}
    \end{tikzpicture}


\caption{RQ3 Results of MAPE}
\label{fig:RQ3_MAPE}
\end{figure}

==> Figures/rq1.1_res.tex <==
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}


\begin{figure}[t]


\subfloat{
        \raisebox{6.8em}{
        \scalebox{1}{
        \begin{tikzpicture}
        
        \begin{customlegend}[legend entries={Improved and significant,Improved but insignificant,Identical with origin},legend style={at={(100,100)},anchor=center,font=\tiny,nodes={scale=1, transform shape},draw=none,fill=none,},]       
        \addlegendimage{black,fill=red!50,area legend}
        \addlegendimage{black,fill=red!20,area legend}
        \addlegendimage{black,fill=blue!30,area legend}
    
        \end{customlegend}
        \end{tikzpicture}
        }
    }
}
\hspace{-13mm}
\setcounter{subfigure}{0}
\subfloat[PERF. results]{
\centering
    \scalebox{0.45}{
    \begin{tikzpicture}
      \pie[rotate=120, text=black,color={red!50, red!20, blue!30},explode = 0.1, sum = auto, scale=1]
      {93, 63, 35}
      % \legend{Same, Different and significant, Different and not significant}
    \end{tikzpicture}
    }
}
\hspace{-5mm}
\subfloat[EFF. results]{
\centering
    \scalebox{0.45}{
    \begin{tikzpicture}
      \pie[rotate=120, text=black, color={red!50, red!20, blue!30},explode = 0.1, sum = auto, scale=1]
      {70, 85, 36}
      % \legend{Same, Different and significant, Different and not significant}
    \end{tikzpicture}
    }
}



\caption{The count on the pairwise comparison results between original SMBO and thes best SMBO with model replaced. There are overall 192 cases (24 systems $\times$ 8 types of SMBO).}
\label{fig:RQ1_sum}
\end{figure}


% 63 35 93
% 85 36 70

==> Lessons_Gained.tex <==


\section{Lessons Learned and Opportunities}

\label{sec:lessons}
In this segment, we explore the practical implications of our discoveries for researcher in the field, considering the lessons gained and potential future opportunities identified.


\begin{itemize}
    \item \textit{\textbf{Lesson 1:} Overall, SMBO with model selection outperforms MFO.}
\end{itemize}



In the comparison of RQ1.1, SMBO with model selection shows a significant advantage with 15 out of 18 in performance and 18 out of 21 in efficiency, making it a more appealing method. An unexpected finding is that within all MFO, configurations outperforming those with model selection are all classified as \texttt{BestConfig}. This suggests that \texttt{BestConfig} has a substantial advantage in certain systems, potentially surpassing SMBO with model replacement.

\begin{itemize}
    \item \textit{\textbf{Lesson 2.1:} For deterministic SMBO, if budget and time permit, it is recommended to try all models. If only a subset of models can be explored, we recommend resorting to classic models like RF or GP to guide sampling.}
    \item \textit{\textbf{Lesson 2.2:} For deterministic SMBO, if your target is performance, use models with higher accuracy. If your goal is efficiency, the high model accuracy can be harmful, and trying all model is low returns and use classic models (GP or RF) is OK.}    
\end{itemize}


Through RQ1.2, we learn that, for most systems, selecting the appropriate model in SMBO contributes to finding better results more efficiently. However, from RQ2.1, we know that only base on accuracy to pick the best and worst model is not completely correct. Therefore, we further explore the accuracy impact from RQ3.1, and it is evident that selecting models based on accuracy may lead to worse performance or efficiency. Considering the difference between performance and efficiency, we find a higher negative correlation within efficiency. Therefore, we reach the conclusion that opting for higher-precision models holds a stronger potential for achieving superior performance outcomes, especially if one strives for optimal performance. However, if your target is efficiency, relying on accuracy, especially using MAPE as a model accuracy measure, may have a negative impact to your optimization results. In this situation, model accuracy is somehow useless.

\begin{itemize}
    \item \textit{\textbf{Lesson 3:} For specific systems, if using BMBO, it is advisable to use µRD as the accuracy metric and select the model with the highest µRD.}
\end{itemize}


By addressing RQ1.1, it is evident that replacing real space with models to expedite optimization can potentially detract from performance but occasionally enhance efficiency. To determine the optimal model selection, RQ2.2 and RQ3.2 provide insights: for BMBO, performance exhibits a substantial positive correlation with accuracy, while efficiency also correlates positively but to a lesser degree. Notably, this positive correlation is more pronounced in µRD. Consequently, selecting models with superior µRD appears to be a rational approach.

\begin{itemize}
    \item \textit{\textbf{Lesson 4:} To make progress by changing the model, at least improve or reduce accuracy under the guidance of Figure~\ref{fig:RQ4_MAPE} and Figure~\ref{fig:RQ4_rank}.}
\end{itemize}

Throughout RQ4, we explore how to change the model can bring significant results improvement.

\begin{itemize}
    \item \textit{\textbf{Lesson 5:} In the SBSE field, compared to using MAPE as a measure of model accuracy, we recommend using rank metric such as µRD as the accuracy metric or considering both simultaneously.}
\end{itemize}


In RQ2 and RQ3, both BMBO and SMBO demonstrate a notable positive correlation between accuracy and results. This positive correlation is stronger when µRD is used as the metric compared to MAPE. This indicates that µRD aligns better with the software engineering when measuring results. When predicting software performance, some researchers solely concentrate on absolute accuracy metrics like MAPE and MSE, which may introduce potential threats. We advise researchers to optimize not only MAPE but also consider relative accuracy differences, specifically the ranking disparities among various configurations in SBSE. This finding also aligns with our intuition: as we seek optimal configurations, each sample relies on model comparisons for selection. Therefore, the higher the accuracy of ranking correctness, the better the outcomes.

% The aforementioned lessons expose the essential guidance for practitioners to take into account when choosing SMBO or MFO as the optimization method. In addition, the lessons also reveals several potential future research avenues in this area. These include:
The aforementioned lessons provide practitioners with crucial guidance to consider when selecting the optimization method. Furthermore, they also unveil numerous potential avenues for future research in this field, including:


==> Tables/RQ2/RQ2_MFO_old.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\caption{A count summary of RQ2 match results}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}l}
\toprule

\textbf{Optimization} &\textbf{Target} & \textbf{Metric}  & \textbf{Best Match} & \textbf{Worst Match} & \textbf{All Match} & \textbf{Match Result}  \\ 
\midrule
MFO&PERF. & MAPE & 94 & 58 & 152 & 41.08\%\\ 
\rowcolor{steel!10}MFO&PERF. & µRD & 93 & 87 & 180 & 48.65\%\ \\ 
MFO&EFF. & MAPE & 31 & 50 & 81 & 21.89\%\ \\ 
\rowcolor{steel!10}MFO&EFF. & µRD & 38 & 63 & 101 & 27.30\%\ \\ 
SMBO&PERF. & MAPE & 51 & 49 & 100 & 20.16\%\\ 
\rowcolor{steel!10}SMBO&PERF. & µRD & 58 & 60 & 118 & 23.79\%\ \\ 
SMBO&EFF. & MAPE & 27 & 40 & 67 & 13.51\%\ \\ 
\rowcolor{steel!10}SMBO&EFF. & µRD & 20 & 54 & 74 & 14.92\%\ \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:rq1_MFO}
\end{table*}

==> Tables/RQ2/rq2_MFO_Eff.tex <==
\begin{table*}[t!]
\caption{The best and worst results of EFF. and MAPE/µRD in BMBO. Formats are the same as Table~\ref{tb:rq2_SMBO_perf}.}
% (DaL/DaL means the first is based on Efficiency while the latter is based on accuracy). Abbreviation restricted to at most 3 words for model: DeepPerf-DeP, HINNPerf-HIP, SPLConquer-SPL, DCTART-DCT. Systems use textsc while models/optimizers use texttt effect.}
\label{tb:rq2_MFO_eff}
\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{19}{c}{\textbf{(a) MAPE and Efficiency}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BestConfig}}}&\multicolumn{2}{c|}{\textbf{\texttt{Irace}}}&\multicolumn{2}{c|}{\textbf{\texttt{GGA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ParamILS}}}&\multicolumn{2}{c|}{\textbf{\texttt{R\_search}}}&\multicolumn{2}{c|}{\textbf{\texttt{GA}}}&\multicolumn{2}{c|}{\textbf{\texttt{SWAY}}}&\multicolumn{2}{c|}{\textbf{\texttt{ConEx}}}&\multicolumn{2}{c}{\textbf{\texttt{E\_search}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule


%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\

\textsc{Brotli}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DaL}&\texttt{DeP/SVR}\\
\textsc{LLVM}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{HIP/RF}&\texttt{SVR/GP}\\
\textsc{Lrzip}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/RF}&\texttt{SPL/LR}\\
\textsc{xgboost}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}\\
\textsc{noc-CM-log}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{DeepArch}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/SPL}\\
\textsc{BDBC}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{DCT/DT}&\texttt{HIP/LR}\\
\textsc{HSQLDB}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{RF/DaL}&\texttt{SPL/GP}\\
\textsc{DConvert}&\texttt{DeP/RF}&\texttt{DT/SVR}&\texttt{DaL/RF}&\texttt{DCT/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\texttt{DeP/SVR}&\texttt{DCT/RF}&\texttt{SPL/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{7z}&\texttt{RF/DT}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{GP/LR}&\texttt{DaL/DT}&\texttt{SVR/LR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{SPL/LR}&\texttt{DaL/DT}&\texttt{GP/LR}&\texttt{RF/DT}&\texttt{SVR/LR}&\texttt{DaL/DT}&\texttt{GP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Apache}&\texttt{SPL/RF}&\texttt{DT/DeP}&\texttt{SPL/RF}&\texttt{DaL/DeP}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/RF}&\texttt{DT/DeP}&\texttt{DeP/RF}&\texttt{SVR/DeP}&\texttt{SPL/RF}&\texttt{GP/DeP}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/RF}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HSMGP}&\texttt{DaL/HIP}&\texttt{SPL/LR}&\texttt{RF/HIP}&\texttt{DeP/LR}&\texttt{RF/HIP}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DCT/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SPL/LR}&\texttt{RF/HIP}&\texttt{GP/LR}&\texttt{LR/HIP}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MongoDB}&\texttt{GP/LR}&\texttt{SPL/SVR}&\texttt{SVR/LR}&\texttt{GP/SVR}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DCT/SVR}&\texttt{DCT/LR}&\texttt{SPL/SVR}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{PostgreSQL}&\texttt{DeP/RF}&\texttt{DaL/DeP}&\texttt{LR/RF}&\texttt{HIP/DeP}&\texttt{HIP/RF}&\texttt{DT/DeP}&\texttt{DeP/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\texttt{SPL/RF}&\texttt{HIP/DeP}&\texttt{DaL/RF}&\texttt{GP/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{ExaStencils}&\texttt{DaL/RF}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{DeP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/RF}&\texttt{GP/SVR}&\texttt{DCT/RF}&\texttt{GP/SVR}&\texttt{DeP/RF}&\texttt{GP/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{kanzi}&\texttt{DeP/RF}&\texttt{DT/LR}&\texttt{GP/RF}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{SVR/RF}&\texttt{DaL/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{jump3r}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/LR}&\texttt{LR/RF}&\texttt{SPL/LR}&\texttt{SVR/RF}&\texttt{SPL/LR}&\texttt{SVR/RF}&\texttt{DT/LR}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DT/RF}&\texttt{DeP/LR}&\texttt{SVR/RF}&\texttt{SPL/LR}&\texttt{SVR/RF}&\texttt{GP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MariaDB}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{LR/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{SPL/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{polly}&\texttt{GP/RF}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/LR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{GP/RF}&\texttt{HIP/LR}&\texttt{GP/RF}&\texttt{DT/LR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SQL}&\texttt{DeP/RF}&\texttt{DT/SPL}&\texttt{SVR/RF}&\texttt{LR/SPL}&\texttt{DeP/RF}&\texttt{LR/SPL}&\texttt{GP/RF}&\texttt{DT/SPL}&\texttt{DT/RF}&\texttt{LR/SPL}&\texttt{LR/RF}&\texttt{DT/SPL}&\texttt{GP/RF}&\texttt{DCT/SPL}&\texttt{LR/RF}&\texttt{DCT/SPL}&\texttt{-/-}&\texttt{-/-}\\
\textsc{vp9}&\texttt{DeP/DT}&\texttt{DT/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{RF/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Spark}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/RF}&\texttt{DaL/GP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{LR/RF}&\texttt{DeP/GP}&\texttt{DCT/RF}&\texttt{DaL/GP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{DT/RF}&\texttt{SPL/GP}&\texttt{DaL/RF}&\texttt{LR/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HIPAcc}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\texttt{GP/SVR}&\texttt{RF/DT}&\texttt{LR/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Redis}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{HIP/DeP}&\texttt{DT/RF}&\texttt{SVR/DeP}&\texttt{HIP/RF}&\texttt{SVR/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\texttt{GP/DeP}&\texttt{DCT/RF}&\texttt{DaL/DeP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{storm}&\texttt{DeP/RF}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{SPL/RF}&\texttt{RF/DT}&\texttt{LR/RF}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/DT}&\texttt{DaL/RF}&\texttt{SPL/DT}&\texttt{GP/RF}&\texttt{DeP/DT}&\texttt{SVR/RF}&\texttt{LR/DT}&\texttt{SPL/RF}&\texttt{DaL/DT}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SaC}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/RF}&\texttt{DeP/SVR}&\texttt{DT/RF}&\texttt{LR/SVR}&\texttt{DT/RF}&\texttt{DeP/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Hadoop}&\texttt{DT/RF}&\texttt{GP/DeP}&\texttt{SVR/RF}&\texttt{LR/DeP}&\texttt{DCT/RF}&\texttt{HIP/DeP}&\texttt{DaL/RF}&\texttt{HIP/DeP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{DT/DeP}&\texttt{DaL/RF}&\texttt{RF/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Tomcat}&\texttt{DCT/RF}&\texttt{SVR/DeP}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\texttt{GP/RF}&\texttt{RF/DeP}&\texttt{DCT/RF}&\texttt{RF/DeP}&\texttt{DaL/RF}&\texttt{HIP/DeP}&\texttt{DCT/RF}&\texttt{DT/DeP}&\texttt{DCT/RF}&\texttt{SPL/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{JavaGC}&\texttt{DeP/RF}&\texttt{SVR/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\texttt{HIP/RF}&\texttt{GP/SPL}&\texttt{DCT/RF}&\texttt{SVR/SPL}&\texttt{DT/RF}&\texttt{SVR/SPL}&\texttt{DaL/RF}&\texttt{DeP/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}&\texttt{-/-}&\texttt{-/-}\\

% 23 37 155 169
% 1 9 31 39






\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{19}{c}{}\\

\multicolumn{19}{c}{\textbf{(b) µRD and Efficiency}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BestConfig}}}&\multicolumn{2}{c|}{\textbf{\texttt{Irace}}}&\multicolumn{2}{c|}{\textbf{\texttt{GGA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ParamILS}}}&\multicolumn{2}{c|}{\textbf{\texttt{R\_search}}}&\multicolumn{2}{c|}{\textbf{\texttt{GA}}}&\multicolumn{2}{c|}{\textbf{\texttt{SWAY}}}&\multicolumn{2}{c|}{\textbf{\texttt{ConEx}}}&\multicolumn{2}{c}{\textbf{\texttt{E\_search}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule

%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\
\textsc{Brotli}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{LLVM}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}\\
\textsc{Lrzip}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\cellcolor{steel!30}\texttt{SPL/SPL}\\
\textsc{xgboost}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}\\
\textsc{noc-CM-log}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/RF}&\texttt{GP/DeP}\\
\textsc{DeepArch}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/SVR}\\
\textsc{BDBC}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{DCT/DT}&\texttt{HIP/GP}\\
\textsc{HSQLDB}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/GP}\\
\textsc{DConvert}&\texttt{DeP/RF}&\texttt{DT/SVR}&\texttt{DaL/RF}&\texttt{DCT/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\texttt{DeP/SVR}&\texttt{DCT/RF}&\texttt{SPL/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{7z}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{GP/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{LR/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{SPL/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Apache}&\texttt{SPL/LR}&\texttt{DT/DeP}&\texttt{SPL/LR}&\texttt{DaL/DeP}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DT/DeP}&\texttt{DeP/LR}&\texttt{SVR/DeP}&\texttt{SPL/LR}&\texttt{GP/DeP}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HSMGP}&\texttt{DaL/HIP}&\texttt{SPL/SVR}&\texttt{RF/HIP}&\texttt{DeP/SVR}&\texttt{RF/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SPL/SVR}&\texttt{RF/HIP}&\texttt{GP/SVR}&\texttt{LR/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MongoDB}&\texttt{GP/RF}&\texttt{SPL/SVR}&\texttt{SVR/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\texttt{DCT/SVR}&\texttt{DCT/RF}&\texttt{SPL/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{PostgreSQL}&\texttt{DeP/DT}&\texttt{DaL/SVR}&\texttt{LR/DT}&\texttt{HIP/SVR}&\texttt{HIP/DT}&\texttt{DT/SVR}&\texttt{DeP/DT}&\texttt{DT/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{SPL/DT}&\texttt{HIP/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{ExaStencils}&\texttt{DaL/RF}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{DeP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/RF}&\texttt{GP/SVR}&\texttt{DCT/RF}&\texttt{GP/SVR}&\texttt{DeP/RF}&\texttt{GP/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{kanzi}&\texttt{DeP/RF}&\texttt{DT/GP}&\texttt{GP/RF}&\texttt{RF/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\texttt{SVR/RF}&\texttt{DaL/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{jump3r}&\texttt{RF/SVR}&\texttt{DeP/GP}&\texttt{LR/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/GP}&\texttt{DT/SVR}&\texttt{DeP/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MariaDB}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{LR/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{SPL/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{polly}&\texttt{GP/RF}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/LR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{GP/RF}&\texttt{HIP/LR}&\texttt{GP/RF}&\texttt{DT/LR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SQL}&\texttt{DeP/RF}&\texttt{DT/SPL}&\texttt{SVR/RF}&\texttt{LR/SPL}&\texttt{DeP/RF}&\texttt{LR/SPL}&\texttt{GP/RF}&\texttt{DT/SPL}&\texttt{DT/RF}&\texttt{LR/SPL}&\texttt{LR/RF}&\texttt{DT/SPL}&\texttt{GP/RF}&\texttt{DCT/SPL}&\texttt{LR/RF}&\texttt{DCT/SPL}&\texttt{-/-}&\texttt{-/-}\\
\textsc{vp9}&\texttt{DeP/DT}&\texttt{DT/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{RF/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Spark}&\texttt{LR/RF}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DaL/SVR}&\texttt{LR/RF}&\texttt{GP/SVR}&\texttt{LR/RF}&\texttt{DeP/SVR}&\texttt{DCT/RF}&\texttt{DaL/SVR}&\texttt{DCT/RF}&\texttt{GP/SVR}&\texttt{DT/RF}&\texttt{SPL/SVR}&\texttt{DaL/RF}&\texttt{LR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HIPAcc}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\texttt{GP/SVR}&\texttt{RF/DT}&\texttt{LR/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Redis}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{HIP/DeP}&\texttt{DT/RF}&\texttt{SVR/DeP}&\texttt{HIP/RF}&\texttt{SVR/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\texttt{GP/DeP}&\texttt{DCT/RF}&\texttt{DaL/DeP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{storm}&\texttt{DeP/RF}&\texttt{DT/DeP}&\texttt{SPL/RF}&\texttt{RF/DeP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\texttt{SPL/DeP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{LR/DeP}&\texttt{SPL/RF}&\texttt{DaL/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SaC}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\texttt{SVR/DeP}&\texttt{DCT/RF}&\texttt{SVR/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{LR/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{SVR/DeP}&\texttt{DCT/RF}&\texttt{SVR/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Hadoop}&\texttt{DT/RF}&\texttt{GP/DeP}&\texttt{SVR/RF}&\texttt{LR/DeP}&\texttt{DCT/RF}&\texttt{HIP/DeP}&\texttt{DaL/RF}&\texttt{HIP/DeP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{DT/DeP}&\texttt{DaL/RF}&\texttt{RF/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Tomcat}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SVR/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\texttt{GP/RF}&\texttt{RF/SVR}&\texttt{DCT/RF}&\texttt{RF/SVR}&\texttt{DaL/RF}&\texttt{HIP/SVR}&\texttt{DCT/RF}&\texttt{DT/SVR}&\texttt{DCT/RF}&\texttt{SPL/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{JavaGC}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{HIP/DT}&\texttt{GP/SVR}&\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{DeP/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\

%28 49 143 164
%3 6 34 37


\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ2/rq2_MFO_Perf.tex <==
\begin{table*}[t!]
\caption{The best and worst results of PERF. and MAPE/µRD in BMBO. Formats are the same as Table~\ref{tb:rq2_SMBO_perf}.}
\label{tb:rq2_MFO_perf}
\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{19}{c}{\textbf{(a) MAPE and Performance}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BestConfig}}}&\multicolumn{2}{c|}{\textbf{\texttt{Irace}}}&\multicolumn{2}{c|}{\textbf{\texttt{GGA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ParamILS}}}&\multicolumn{2}{c|}{\textbf{\texttt{R\_search}}}&\multicolumn{2}{c|}{\textbf{\texttt{GA}}}&\multicolumn{2}{c|}{\textbf{\texttt{SWAY}}}&\multicolumn{2}{c|}{\textbf{\texttt{ConEx}}}&\multicolumn{2}{c}{\textbf{\texttt{E\_search}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule


%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\

\textsc{Brotli}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DaL}&\texttt{GP/SVR}\\
\textsc{LLVM}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/GP}\\
\textsc{Lrzip}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}\\
\textsc{xgboost}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SPL}\\
\textsc{noc-CM-log}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{DeepArch}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}\\
\textsc{BDBC}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{RF/DT}&\texttt{DeP/LR}\\
\textsc{HSQLDB}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{RF/DaL}&\texttt{DT/GP}\\
\textsc{DConvert}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{7z}&\texttt{RF/DT}&\texttt{DeP/LR}&\texttt{DaL/DT}&\texttt{SVR/LR}&\texttt{RF/DT}&\texttt{DeP/LR}&\texttt{RF/DT}&\texttt{SVR/LR}&\texttt{DaL/DT}&\texttt{SPL/LR}&\texttt{DaL/DT}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{SVR/LR}&\texttt{DaL/DT}&\texttt{GP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Apache}&\texttt{SPL/RF}&\texttt{DaL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HSMGP}&\texttt{DaL/HIP}&\texttt{DeP/LR}&\texttt{RF/HIP}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SPL/LR}&\texttt{DaL/HIP}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MongoDB}&\texttt{HIP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SPL/SVR}&\texttt{HIP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{PostgreSQL}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DCT/RF}&\texttt{SVR/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\texttt{GP/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{ExaStencils}&\texttt{LR/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{kanzi}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{jump3r}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/RF}&\texttt{SPL/LR}&\texttt{SVR/RF}&\texttt{SPL/LR}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/RF}&\texttt{HIP/LR}&\texttt{SVR/RF}&\texttt{GP/LR}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/RF}&\texttt{GP/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MariaDB}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{polly}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{DaL/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SQL}&\texttt{SVR/RF}&\texttt{DeP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SPL}&\texttt{DeP/RF}&\texttt{HIP/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SPL}&\texttt{-/-}&\texttt{-/-}\\
\textsc{vp9}&\texttt{RF/DT}&\texttt{LR/SVR}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Spark}&\texttt{LR/RF}&\texttt{DT/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\texttt{HIP/RF}&\texttt{DCT/GP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HIPAcc}&\texttt{HIP/DT}&\texttt{LR/SVR}&\texttt{DaL/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Redis}&\texttt{DaL/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{storm}&\texttt{DaL/RF}&\texttt{DeP/DT}&\texttt{DaL/RF}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/DT}&\texttt{DaL/RF}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/DT}&\texttt{DaL/RF}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/DT}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SaC}&\texttt{LR/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/SVR}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\texttt{DCT/RF}&\texttt{SPL/SVR}&\texttt{DT/RF}&\texttt{DeP/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Hadoop}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\texttt{DeP/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Tomcat}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{DCT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{JavaGC}&\texttt{LR/RF}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{DaL/RF}&\texttt{SVR/SPL}&\texttt{DT/RF}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/SPL}&\texttt{-/-}&\texttt{-/-}\\

%63 44 92 73
%29 18 22 11




\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{19}{c}{}\\

\multicolumn{19}{c}{\textbf{(b) µRD and Performance}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BestConfig}}}&\multicolumn{2}{c|}{\textbf{\texttt{Irace}}}&\multicolumn{2}{c|}{\textbf{\texttt{GGA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ParamILS}}}&\multicolumn{2}{c|}{\textbf{\texttt{R\_search}}}&\multicolumn{2}{c|}{\textbf{\texttt{GA}}}&\multicolumn{2}{c|}{\textbf{\texttt{SWAY}}}&\multicolumn{2}{c|}{\textbf{\texttt{ConEx}}}&\multicolumn{2}{c}{\textbf{\texttt{E\_search}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule

%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\
\textsc{Brotli}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\texttt{GP/DeP}\\
\textsc{LLVM}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}\\
\textsc{Lrzip}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/DT}&\texttt{LR/SPL}\\
\textsc{xgboost}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SVR}\\
\textsc{noc-CM-log}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{SVR/RF}&\texttt{GP/DeP}\\
\textsc{DeepArch}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}\\
\textsc{BDBC}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{RF/DT}&\texttt{DeP/GP}\\
\textsc{HSQLDB}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\texttt{-/-}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/GP}\\
\textsc{DConvert}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{7z}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{SPL/SVR}&\texttt{DaL/DT}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Apache}&\texttt{SPL/LR}&\texttt{DaL/DeP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/LR}&\texttt{SPL/DeP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HSMGP}&\texttt{DaL/HIP}&\texttt{DeP/SVR}&\texttt{RF/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SPL/SVR}&\texttt{DaL/HIP}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MongoDB}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\texttt{SPL/SVR}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{PostgreSQL}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{HIP/SVR}&\texttt{GP/DT}&\texttt{SPL/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{ExaStencils}&\texttt{LR/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{kanzi}&\texttt{SVR/RF}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{jump3r}&\texttt{DaL/SVR}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{MariaDB}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{polly}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{DaL/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SQL}&\texttt{SVR/RF}&\texttt{DeP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SPL}&\texttt{DeP/RF}&\texttt{HIP/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\texttt{DaL/RF}&\texttt{GP/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SPL}&\texttt{-/-}&\texttt{-/-}\\
\textsc{vp9}&\texttt{RF/DT}&\texttt{LR/SVR}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Spark}&\texttt{LR/RF}&\texttt{DT/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\texttt{DCT/SVR}&\texttt{DaL/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{HIPAcc}&\texttt{HIP/DT}&\texttt{LR/SVR}&\texttt{DaL/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Redis}&\texttt{DaL/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{storm}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{SaC}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/DeP}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DCT/RF}&\texttt{SPL/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Hadoop}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/DeP}&\texttt{DeP/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\texttt{-/-}&\texttt{-/-}\\
\textsc{Tomcat}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\texttt{DaL/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\texttt{DeP/RF}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\
\textsc{JavaGC}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{DeP/SVR}&\texttt{RF/DT}&\texttt{SPL/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{-/-}&\texttt{-/-}\\

%58 64 72 78
%24 14 26 16



\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ2/rq2_SMBO_Eff.tex <==
\begin{table*}[t!]
\caption{The best and worst results of EFF. and MAPE/µRD in SMBO. Formats are the same as Table~\ref{tb:rq2_SMBO_perf}.}
% (DaL/DaL means the first is based on Efficiency while the latter is based on accuracy). Abbreviation restricted to at most 3 words for model: DeepPerf-DeP, HINNPerf-HIP, SPLConquer-SPL, DCTART-DCT. Systems use textsc while models/optimizers use texttt effect.}
\label{tb:rq2_SMBO_eff}
\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{17}{c}{\textbf{(a) MAPE and Efficiency}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BOCA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ATConf}}}&\multicolumn{2}{c|}{\textbf{\texttt{FLASH}}}&\multicolumn{2}{c|}{\textbf{\texttt{OtterTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ResTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ROBOTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{SMAC}}}&\multicolumn{2}{c}{\textbf{\texttt{Tuneful}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule


%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\

\textsc{Brotli}&\texttt{GP/RF}&\texttt{DeP/HIP}&\texttt{LR/DeP}&\texttt{RF/GP}&\texttt{LR/DT}&\texttt{GP/SVR}&\texttt{SVR/DCT}&\texttt{DeP/SVR}&\texttt{LR/RF}&\texttt{SVR/HIP}&\texttt{DaL/RF}&\texttt{SVR/HIP}&\texttt{GP/DCT}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\texttt{SVR/HIP}\\
\textsc{LLVM}&\texttt{HIP/RF}&\texttt{SVR/GP}&\texttt{SPL/LR}&\texttt{RF/GP}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DeP/SVR}&\texttt{GP/LR}&\texttt{DCT/SVR}&\texttt{SPL/HIP}&\texttt{DT/GP}&\texttt{GP/RF}&\texttt{SVR/GP}&\texttt{GP/LR}&\texttt{DT/GP}\\
\textsc{Lrzip}&\texttt{DaL/SPL}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/HIP}&\texttt{SVR/DT}&\texttt{RF/LR}&\texttt{SVR/DT}&\texttt{DT/LR}&\texttt{SVR/SPL}&\texttt{DeP/HIP}&\texttt{GP/RF}&\texttt{DCT/HIP}&\texttt{GP/DT}&\texttt{DT/LR}&\texttt{HIP/RF}&\texttt{DCT/HIP}\\
\textsc{xgboost}&\texttt{RF/DT}&\texttt{GP/SVR}&\texttt{SPL/RF}&\texttt{DCT/DeP}&\texttt{RF/HIP}&\texttt{GP/SVR}&\texttt{DeP/DT}&\texttt{SVR/SPL}&\texttt{GP/RF}&\texttt{DT/SPL}&\texttt{GP/RF}&\texttt{RF/GP}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{noc-CM-log}&\texttt{GP/DCT}&\texttt{DaL/SPL}&\texttt{LR/RF}&\texttt{GP/SVR}&\texttt{DeP/DT}&\texttt{DaL/GP}&\texttt{SVR/DT}&\texttt{DaL/GP}&\texttt{DeP/DT}&\texttt{SPL/GP}&\texttt{SPL/RF}&\texttt{DCT/GP}&\texttt{GP/DT}&\texttt{DaL/LR}&\texttt{HIP/DT}&\texttt{DCT/GP}\\
\textsc{DeepArch}&\texttt{DeP/DT}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DT/DeP}&\texttt{RF/SPL}&\texttt{GP/SVR}&\texttt{DCT/RF}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DCT/SPL}&\texttt{GP/RF}&\texttt{DaL/DeP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\texttt{DT/DeP}\\
\textsc{BDBC}&\texttt{DeP/DCT}&\texttt{DT/HIP}&\texttt{LR/DaL}&\texttt{DaL/DeP}&\texttt{RF/DaL}&\texttt{SVR/LR}&\texttt{RF/DT}&\texttt{SVR/LR}&\texttt{LR/DaL}&\texttt{RF/HIP}&\texttt{LR/DaL}&\texttt{DT/SVR}&\texttt{GP/DT}&\texttt{RF/LR}&\texttt{LR/DaL}&\texttt{RF/DeP}\\
\textsc{HSQLDB}&\texttt{GP/DCT}&\texttt{DT/SVR}&\texttt{SPL/DT}&\texttt{DeP/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/DT}&\texttt{DeP/SVR}&\texttt{GP/HIP}&\texttt{DeP/GP}&\texttt{GP/DT}&\texttt{DCT/GP}&\texttt{LR/DT}&\texttt{DCT/SVR}\\
\textsc{DConvert}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/DeP}&\texttt{DCT/GP}&\texttt{SVR/DeP}&\texttt{DCT/SPL}&\texttt{GP/DCT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/DeP}&\texttt{RF/GP}\\
\textsc{7z}&\texttt{DaL/RF}&\texttt{DT/SVR}&\texttt{DeP/RF}&\texttt{DT/HIP}&\texttt{DaL/DCT}&\texttt{GP/SVR}&\texttt{DaL/DCT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/GP}&\texttt{RF/DT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}\\
\textsc{Apache}&\texttt{RF/DCT}&\texttt{DeP/GP}&\texttt{SPL/DCT}&\texttt{DT/SVR}&\texttt{GP/DCT}&\texttt{RF/SVR}&\texttt{GP/RF}&\texttt{DeP/SVR}&\texttt{SVR/DCT}&\texttt{DeP/GP}&\texttt{GP/DCT}&\texttt{DT/HIP}&\texttt{GP/RF}&\texttt{DCT/GP}&\texttt{SVR/DCT}&\texttt{DeP/GP}\\
\textsc{HSMGP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DT/SVR}&\texttt{SPL/RF}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/HIP}&\texttt{DCT/DeP}&\texttt{SPL/DaL}&\texttt{DeP/LR}&\texttt{SPL/DT}&\texttt{DCT/SVR}&\texttt{LR/HIP}&\texttt{DCT/DeP}\\
\textsc{MongoDB}&\texttt{RF/DCT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{DT/GP}&\texttt{SPL/LR}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DT/DeP}\\
\textsc{PostgreSQL}&\texttt{LR/SVR}&\texttt{DCT/DeP}&\texttt{GP/DT}&\texttt{DCT/DeP}&\texttt{GP/DaL}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\texttt{DCT/DT}&\texttt{DeP/GP}&\texttt{DaL/HIP}&\texttt{DeP/GP}&\texttt{GP/SVR}&\texttt{DCT/DeP}&\texttt{SPL/DT}&\texttt{DeP/GP}\\
\textsc{ExaStencils}&\texttt{DCT/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{LR/GP}&\texttt{GP/RF}&\texttt{DeP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/GP}\\
\textsc{kanzi}&\texttt{LR/RF}&\texttt{DT/LR}&\texttt{GP/RF}&\texttt{RF/HIP}&\texttt{RF/DeP}&\texttt{GP/LR}&\texttt{RF/DCT}&\texttt{GP/LR}&\texttt{SVR/RF}&\texttt{DT/HIP}&\texttt{SVR/RF}&\texttt{DeP/HIP}&\texttt{SPL/RF}&\texttt{DT/LR}&\texttt{GP/RF}&\texttt{DCT/HIP}\\
\textsc{jump3r}&\texttt{GP/RF}&\texttt{DT/LR}&\texttt{SPL/RF}&\texttt{DCT/HIP}&\texttt{DeP/SPL}&\texttt{SVR/LR}&\texttt{GP/DT}&\texttt{DCT/LR}&\texttt{GP/RF}&\texttt{RF/GP}&\texttt{SVR/RF}&\texttt{DaL/GP}&\texttt{HIP/DT}&\texttt{DT/LR}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{MariaDB}&\texttt{LR/DT}&\texttt{RF/SVR}&\texttt{SPL/DaL}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DeP/SVR}&\texttt{SPL/DT}&\texttt{DeP/SVR}&\texttt{SPL/DeP}&\texttt{RF/SVR}&\texttt{GP/DeP}&\texttt{DCT/GP}&\texttt{GP/DT}&\texttt{DeP/SVR}&\texttt{SPL/DeP}&\texttt{DeP/GP}\\
\textsc{polly}&\texttt{DCT/DT}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{DCT/DCT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{RF/SVR}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/GP}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/SVR}&\texttt{SPL/GP}\\
\textsc{SQL}&\texttt{DT/SVR}&\texttt{DeP/LR}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{DeP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/LR}&\texttt{GP/SVR}&\texttt{DaL/LR}&\texttt{SVR/RF}&\texttt{DCT/LR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/SVR}&\texttt{DCT/LR}\\
\textsc{vp9}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{GP/DCT}&\texttt{DT/SVR}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{GP/DCT}&\texttt{SPL/GP}&\texttt{DeP/HIP}&\texttt{DCT/GP}&\texttt{SPL/DT}&\texttt{GP/SVR}&\texttt{GP/DCT}&\texttt{SPL/GP}\\
\textsc{Spark}&\texttt{SPL/RF}&\texttt{DaL/SVR}&\texttt{SVR/RF}&\texttt{DeP/SVR}&\texttt{RF/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/DT}&\texttt{DaL/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{DeP/LR}&\texttt{GP/RF}&\texttt{DaL/DeP}&\texttt{GP/RF}&\texttt{DeP/GP}\\
\textsc{HIPAcc}&\texttt{GP/RF}&\texttt{DaL/SVR}&\texttt{SPL/RF}&\texttt{DT/SVR}&\texttt{RF/DaL}&\texttt{DeP/SVR}&\texttt{DCT/HIP}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/DaL}&\texttt{DeP/GP}&\texttt{DaL/RF}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\texttt{DeP/LR}\\
\textsc{Redis}&\texttt{HIP/GP}&\texttt{GP/DeP}&\texttt{LR/DeP}&\texttt{GP/DT}&\texttt{GP/SVR}&\texttt{DaL/DeP}&\texttt{GP/SVR}&\texttt{RF/DeP}&\texttt{HIP/SVR}&\texttt{DaL/GP}&\texttt{SPL/LR}&\texttt{HIP/GP}&\texttt{GP/SVR}&\texttt{SVR/DeP}&\texttt{LR/SVR}&\texttt{DCT/GP}\\
\textsc{storm}&\texttt{GP/RF}&\texttt{SVR/DT}&\texttt{GP/RF}&\texttt{RF/DT}&\texttt{DeP/LR}&\texttt{DaL/RF}&\texttt{SPL/LR}&\texttt{DaL/DT}&\texttt{SPL/RF}&\texttt{HIP/DT}&\texttt{DeP/LR}&\texttt{SPL/DCT}&\texttt{DeP/RF}&\texttt{SVR/DT}&\texttt{LR/RF}&\texttt{GP/DT}\\
\textsc{SaC}&\texttt{DeP/HIP}&\texttt{DT/DeP}&\texttt{DeP/RF}&\texttt{LR/SVR}&\texttt{SPL/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{GP/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{GP/LR}\\
\textsc{Hadoop}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/DeP}&\texttt{SPL/RF}&\texttt{DCT/DeP}&\texttt{LR/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{DT/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{DCT/GP}\\
\textsc{Tomcat}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{HIP/DeP}&\texttt{DCT/RF}&\texttt{SVR/DeP}&\texttt{GP/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{DeP/GP}&\texttt{SPL/RF}&\texttt{DeP/SPL}&\texttt{DaL/RF}&\texttt{LR/DeP}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{JavaGC}&\texttt{LR/RF}&\texttt{DeP/SVR}&\texttt{DaL/RF}&\texttt{GP/HIP}&\texttt{RF/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/RF}&\texttt{DeP/HIP}&\texttt{SPL/RF}&\texttt{DeP/HIP}&\texttt{DaL/RF}&\texttt{GP/LR}\\

%%24 29 163 168
%6 7 33 34







\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{17}{c}{}\\

\multicolumn{17}{c}{\textbf{(b) µRD and Efficiency}}\\

\toprule

\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BOCA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ATConf}}}&\multicolumn{2}{c|}{\textbf{\texttt{FLASH}}}&\multicolumn{2}{c|}{\textbf{\texttt{OtterTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ResTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ROBOTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{SMAC}}}&\multicolumn{2}{c}{\textbf{\texttt{Tuneful}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule

%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\
\textsc{Brotli}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/DaL}&\texttt{RF/DeP}&\texttt{LR/DeP}&\texttt{GP/DCT}&\texttt{SVR/DaL}&\texttt{DeP/SVR}&\texttt{LR/DaL}&\texttt{SVR/DeP}&\texttt{DaL/RF}&\texttt{SVR/DeP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/DaL}&\texttt{SVR/DeP}\\
\textsc{LLVM}&\texttt{HIP/RF}&\texttt{SVR/DeP}&\texttt{SPL/LR}&\texttt{RF/GP}&\texttt{SPL/LR}&\texttt{DeP/DCT}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/SPL}&\texttt{DCT/GP}&\texttt{SPL/HIP}&\texttt{DT/GP}&\texttt{GP/RF}&\texttt{SVR/DeP}&\texttt{GP/LR}&\texttt{DT/GP}\\
\textsc{Lrzip}&\texttt{DaL/DT}&\texttt{HIP/GP}&\texttt{RF/SVR}&\texttt{SPL/LR}&\texttt{SVR/RF}&\texttt{RF/LR}&\texttt{SVR/DT}&\texttt{DT/GP}&\texttt{SVR/HIP}&\texttt{DeP/DCT}&\texttt{GP/DeP}&\texttt{DCT/GP}&\texttt{GP/DT}&\texttt{DT/GP}&\texttt{HIP/SVR}&\texttt{DCT/SPL}\\
\textsc{xgboost}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{SPL/LR}&\texttt{DCT/GP}&\texttt{RF/HIP}&\texttt{GP/SVR}&\texttt{DeP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/LR}&\texttt{DT/SVR}&\texttt{GP/LR}&\texttt{RF/GP}&\texttt{DeP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/HIP}&\texttt{DeP/GP}\\
\textsc{noc-CM-log}&\texttt{GP/RF}&\texttt{DaL/GP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{DeP/DaL}&\texttt{DaL/GP}&\texttt{SVR/RF}&\texttt{DaL/GP}&\texttt{DeP/RF}&\texttt{SPL/GP}&\texttt{SPL/RF}&\texttt{DCT/GP}&\texttt{GP/DT}&\texttt{DaL/GP}&\texttt{HIP/RF}&\texttt{DCT/GP}\\
\textsc{DeepArch}&\texttt{DeP/DT}&\texttt{GP/SVR}&\texttt{GP/LR}&\texttt{DT/GP}&\texttt{RF/HIP}&\texttt{GP/SVR}&\texttt{DCT/HIP}&\texttt{GP/SVR}&\texttt{GP/SPL}&\texttt{DCT/DeP}&\texttt{GP/LR}&\texttt{DaL/GP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\texttt{DT/GP}\\
\textsc{BDBC}&\texttt{DeP/RF}&\texttt{DT/GP}&\texttt{LR/RF}&\texttt{DaL/SVR}&\texttt{RF/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\texttt{SVR/GP}&\texttt{LR/RF}&\texttt{RF/SVR}&\texttt{LR/RF}&\texttt{DT/GP}&\texttt{GP/DT}&\texttt{RF/GP}&\texttt{LR/RF}&\texttt{RF/GP}\\
\textsc{HSQLDB}&\texttt{GP/DT}&\texttt{DT/SVR}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/HIP}&\texttt{DeP/SVR}&\texttt{GP/HIP}&\texttt{DeP/GP}&\texttt{GP/RF}&\texttt{DCT/GP}&\texttt{LR/HIP}&\texttt{DCT/SVR}\\
\textsc{DConvert}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\texttt{DCT/HIP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/DeP}&\texttt{DCT/GP}&\texttt{SVR/DeP}&\texttt{DCT/GP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/RF}&\texttt{RF/GP}\\
\textsc{7z}&\texttt{DaL/RF}&\texttt{DT/SVR}&\texttt{DeP/DaL}&\texttt{DT/DeP}&\texttt{DaL/HIP}&\texttt{GP/SVR}&\texttt{DaL/DT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}\\
\textsc{Apache}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{DT/GP}&\texttt{GP/LR}&\texttt{RF/SVR}&\texttt{GP/LR}&\texttt{DeP/SVR}&\texttt{SVR/DeP}&\texttt{DeP/DCT}&\texttt{GP/DaL}&\texttt{DT/GP}&\texttt{GP/LR}&\texttt{DCT/GP}&\texttt{SVR/DeP}&\texttt{DeP/DCT}\\
\textsc{HSMGP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{DT/SVR}&\texttt{SPL/HIP}&\texttt{DCT/DeP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/HIP}&\texttt{DCT/DeP}&\texttt{SPL/HIP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/HIP}&\texttt{DCT/SVR}&\texttt{LR/HIP}&\texttt{DCT/DeP}\\
\textsc{MongoDB}&\texttt{RF/SPL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/SPL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{DT/DeP}&\texttt{SPL/LR}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DT/DeP}\\
\textsc{PostgreSQL}&\texttt{LR/SPL}&\texttt{DCT/SVR}&\texttt{GP/SPL}&\texttt{DCT/DeP}&\texttt{GP/DaL}&\texttt{DCT/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/GP}&\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/SPL}&\texttt{DCT/SVR}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{ExaStencils}&\texttt{DCT/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{LR/DeP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/DeP}\\
\textsc{kanzi}&\texttt{LR/DeP}&\texttt{DT/GP}&\texttt{GP/SPL}&\texttt{RF/DeP}&\texttt{RF/DeP}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SVR/HIP}&\texttt{DT/DeP}&\texttt{SVR/HIP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\texttt{DT/GP}&\texttt{GP/RF}&\texttt{DCT/DeP}\\
\textsc{jump3r}&\texttt{GP/DaL}&\texttt{DT/DeP}&\texttt{SPL/RF}&\texttt{DCT/DeP}&\texttt{DeP/HIP}&\texttt{SVR/DCT}&\texttt{GP/DaL}&\texttt{DCT/SPL}&\texttt{GP/LR}&\texttt{RF/GP}&\texttt{SVR/RF}&\texttt{DaL/GP}&\texttt{HIP/SVR}&\texttt{DT/DeP}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{MariaDB}&\texttt{LR/RF}&\texttt{RF/DeP}&\texttt{SPL/RF}&\texttt{DCT/SVR}&\texttt{DT/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\texttt{RF/GP}&\texttt{GP/RF}&\texttt{DCT/GP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/RF}&\texttt{DeP/GP}\\
\textsc{polly}&\texttt{DCT/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{HIP/GP}&\texttt{DCT/DaL}&\texttt{SVR/LR}&\texttt{DeP/HIP}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{RF/HIP}&\texttt{SPL/GP}&\texttt{SVR/HIP}&\texttt{HIP/GP}&\texttt{DT/RF}&\texttt{SVR/GP}&\texttt{RF/HIP}&\texttt{SPL/GP}\\
\textsc{SQL}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{DT/DCT}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/DCT}&\texttt{DCT/DeP}&\texttt{GP/SVR}&\texttt{DaL/DCT}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{GP/RF}&\texttt{DeP/GP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DCT/DCT}\\
\textsc{vp9}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/DT}&\texttt{DT/DeP}&\texttt{RF/DT}&\texttt{GP/SVR}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/DT}&\texttt{SPL/GP}&\texttt{DeP/DT}&\texttt{DCT/GP}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/DT}&\texttt{SPL/GP}\\
\textsc{Spark}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{DaL/DeP}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/DaL}&\texttt{DeP/SVR}&\texttt{SVR/DaL}&\texttt{DaL/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{DaL/DeP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{HIPAcc}&\texttt{GP/SPL}&\texttt{DaL/SVR}&\texttt{SPL/RF}&\texttt{DT/DeP}&\texttt{RF/DaL}&\texttt{DeP/SVR}&\texttt{DCT/DaL}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{DeP/GP}&\texttt{DaL/RF}&\texttt{DeP/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{Redis}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/DeP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/RF}&\texttt{DaL/GP}&\texttt{GP/DT}&\texttt{RF/GP}&\texttt{HIP/SVR}&\texttt{DaL/DeP}&\texttt{SPL/RF}&\texttt{HIP/DeP}&\texttt{GP/RF}&\texttt{SVR/GP}&\texttt{LR/DCT}&\texttt{DCT/DeP}\\
\textsc{storm}&\texttt{GP/DT}&\texttt{SVR/DeP}&\texttt{GP/RF}&\texttt{RF/SVR}&\texttt{DeP/DaL}&\texttt{DaL/DeP}&\texttt{SPL/DaL}&\texttt{DaL/DeP}&\texttt{SPL/RF}&\texttt{HIP/SVR}&\texttt{DeP/RF}&\texttt{SPL/GP}&\texttt{DeP/DT}&\texttt{SVR/DeP}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{SaC}&\texttt{DeP/HIP}&\texttt{DT/SVR}&\texttt{DeP/HIP}&\texttt{LR/SVR}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\texttt{HIP/DCT}&\texttt{DeP/SVR}&\texttt{HIP/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/DeP}&\texttt{SPL/DCT}&\texttt{GP/DT}&\texttt{DeP/SVR}&\texttt{DeP/SVR}&\texttt{GP/LR}\\
\textsc{Hadoop}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DCT/DeP}&\texttt{SPL/RF}&\texttt{DCT/DeP}&\texttt{LR/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SVR/RF}&\texttt{DT/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{DCT/DeP}\\
\textsc{Tomcat}&\texttt{GP/LR}&\texttt{HIP/SVR}&\texttt{DCT/RF}&\texttt{SVR/GP}&\texttt{GP/DaL}&\texttt{DeP/SVR}&\texttt{RF/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/RF}&\texttt{DeP/GP}&\texttt{SPL/RF}&\texttt{DeP/GP}&\texttt{DaL/RF}&\texttt{LR/SVR}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{JavaGC}&\texttt{LR/SPL}&\texttt{DeP/SVR}&\texttt{DaL/RF}&\texttt{GP/SVR}&\texttt{RF/HIP}&\texttt{SVR/GP}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{LR/SPL}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/HIP}&\texttt{DeP/GP}&\texttt{SPL/RF}&\texttt{DeP/SVR}&\texttt{DaL/SVR}&\texttt{GP/LR}\\

%17 46 146 175
%7 9 31 33


\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ2/rq2_SMBO_Perf.tex <==
\begin{table*}[t!]
\caption{The best and worst results of PERF. and MAPE/µRD in SMBO (DaL/DaL means the first is based on performance while the latter is based on accuracy). Abbreviation restricted to at most 3 words for model: DeepPerf-DeP, HINNPerf-HIP, SPLConquer-SPL, DCTART-DCT.}
% Systems use textsc while models/optimizers use texttt effect.}
\label{tb:rq2_SMBO_perf}
\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{17}{c}{\textbf{(a) MAPE and Performance}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BOCA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ATConf}}}&\multicolumn{2}{c|}{\textbf{\texttt{FLASH}}}&\multicolumn{2}{c|}{\textbf{\texttt{OtterTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ResTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ROBOTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{SMAC}}}&\multicolumn{2}{c}{\textbf{\texttt{Tuneful}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule


%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\

\textsc{Brotli}&\texttt{DT/RF}&\texttt{DaL/HIP}&\texttt{GP/DeP}&\texttt{RF/GP}&\texttt{DeP/DT}&\texttt{DT/SVR}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{LR/SVR}&\texttt{DaL/RF}&\texttt{SVR/HIP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/HIP}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{SVR/HIP}\\
\textsc{LLVM}&\texttt{HIP/RF}&\texttt{DeP/GP}&\texttt{GP/LR}&\texttt{RF/GP}&\texttt{DT/SPL}&\texttt{DT/SVR}&\texttt{DaL/LR}&\texttt{DeP/SVR}&\texttt{HIP/LR}&\texttt{DCT/SVR}&\texttt{DaL/HIP}&\texttt{SVR/GP}&\texttt{DCT/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{HIP/LR}&\texttt{SVR/GP}\\
\textsc{Lrzip}&\texttt{HIP/SPL}&\texttt{GP/HIP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/HIP}&\texttt{RF/DT}&\texttt{DT/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{GP/LR}&\texttt{RF/SPL}&\texttt{SVR/HIP}&\texttt{DCT/RF}&\texttt{SPL/HIP}&\texttt{RF/DT}&\texttt{GP/LR}&\texttt{GP/RF}&\texttt{LR/HIP}\\
\textsc{xgboost}&\texttt{RF/DT}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{DCT/DeP}&\texttt{DeP/HIP}&\texttt{GP/SVR}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{GP/RF}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/GP}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{GP/SVR}&\texttt{DeP/RF}&\texttt{LR/DeP}\\
\textsc{noc-CM-log}&\texttt{RF/DCT}&\texttt{DaL/SPL}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{DaL/DT}&\texttt{RF/GP}&\texttt{RF/DT}&\texttt{DaL/GP}&\texttt{DeP/DT}&\texttt{SPL/GP}&\texttt{DeP/RF}&\texttt{SVR/GP}&\texttt{DeP/DT}&\texttt{DaL/LR}&\texttt{HIP/DT}&\texttt{SVR/GP}\\
\textsc{DeepArch}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/RF}&\texttt{SPL/DeP}&\texttt{DeP/SPL}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/SPL}&\texttt{HIP/RF}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DaL/SVR}&\texttt{DaL/RF}&\texttt{SVR/DeP}\\
\textsc{BDBC}&\texttt{LR/DCT}&\texttt{RF/HIP}&\texttt{GP/DaL}&\texttt{RF/DeP}&\texttt{DeP/DaL}&\texttt{SVR/LR}&\texttt{DeP/DT}&\texttt{SVR/LR}&\texttt{GP/DaL}&\texttt{SVR/HIP}&\texttt{RF/DaL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DaL/LR}&\texttt{HIP/DaL}&\texttt{SVR/DeP}\\
\textsc{HSQLDB}&\texttt{SPL/DCT}&\texttt{DCT/SVR}&\texttt{GP/DT}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/GP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}\\
\textsc{DConvert}&\texttt{GP/RF}&\texttt{DeP/SVR}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DeP}&\texttt{DT/GP}&\texttt{HIP/DeP}&\texttt{SVR/SPL}&\texttt{RF/DCT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DeP}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{7z}&\texttt{HIP/RF}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{RF/HIP}&\texttt{DeP/DCT}&\texttt{SPL/SVR}&\texttt{DeP/DCT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/GP}&\texttt{DCT/DT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}\\
\textsc{Apache}&\texttt{DaL/SVR}&\texttt{SVR/DEC}&\texttt{DT/SVR}&\texttt{SVR/DEC}&\texttt{LR/GP}&\texttt{GP/DEC}&\texttt{HIP/SVR}&\texttt{SVR/RF}&\texttt{DaL/SVR}&\texttt{SVR/DEC}&\texttt{DT/SPL}&\texttt{SPL/DEC}&\texttt{RF/GP}&\texttt{GP/RF}&\texttt{DaL/SVR}&\texttt{SVR/DEC}\\
\textsc{HSMGP}&\texttt{LR/HIP}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{RF/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/HIP}&\texttt{DCT/DeP}&\texttt{HIP/DaL}&\texttt{SVR/LR}&\texttt{HIP/DT}&\texttt{GP/SVR}&\texttt{GP/HIP}&\texttt{DCT/DeP}\\
\textsc{MongoDB}&\texttt{SPL/DCT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{SVR/GP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{PostgreSQL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/DeP}&\texttt{DaL/DT}&\texttt{SVR/DeP}&\texttt{DeP/DaL}&\texttt{SPL/SVR}&\texttt{DT/RF}&\texttt{GP/DeP}&\texttt{RF/DT}&\texttt{SVR/GP}&\texttt{DaL/HIP}&\texttt{SPL/GP}&\texttt{DCT/SVR}&\texttt{GP/DeP}&\texttt{RF/DT}&\texttt{SVR/GP}\\
\textsc{ExaStencils}&\texttt{DeP/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/SVR}&\texttt{DeP/DaL}&\texttt{GP/LR}&\texttt{DeP/DaL}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{LR/GP}&\texttt{GP/RF}&\texttt{SPL/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/GP}\\
\textsc{kanzi}&\texttt{SPL/RF}&\texttt{RF/LR}&\texttt{SVR/RF}&\texttt{RF/HIP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{GP/LR}&\texttt{GP/RF}&\texttt{DCT/HIP}&\texttt{HIP/RF}&\texttt{SVR/HIP}&\texttt{HIP/RF}&\texttt{GP/LR}&\texttt{SPL/RF}&\texttt{RF/HIP}\\
\textsc{jump3r}&\texttt{GP/RF}&\texttt{RF/LR}&\texttt{GP/RF}&\texttt{SVR/HIP}&\texttt{DeP/SPL}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DeP/LR}&\texttt{GP/RF}&\texttt{RF/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\texttt{SVR/DT}&\texttt{DCT/LR}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{MariaDB}&\texttt{SPL/DT}&\texttt{DaL/SVR}&\texttt{GP/DaL}&\texttt{RF/SVR}&\texttt{SPL/DT}&\texttt{DeP/SVR}&\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/DeP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{SPL/GP}&\texttt{DCT/DT}&\texttt{GP/SVR}&\texttt{DT/DeP}&\texttt{SPL/GP}\\
\textsc{polly}&\texttt{DCT/DT}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/HIP}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{GP/SVR}&\texttt{HIP/DT}&\texttt{SVR/LR}&\texttt{DaL/SVR}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/SVR}&\texttt{SVR/GP}&\texttt{RF/DT}&\texttt{GP/SVR}&\texttt{DaL/SVR}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{SQL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DeP/LR}&\texttt{DeP/SVR}&\texttt{SVR/DT}&\texttt{SPL/DaL}&\texttt{SVR/LR}&\texttt{LR/SVR}&\texttt{DeP/LR}&\texttt{RF/SVR}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/LR}&\texttt{SPL/RF}&\texttt{SVR/DeP}&\texttt{RF/SVR}&\texttt{GP/LR}\\
\textsc{vp9}&\texttt{RF/DCT}&\texttt{GP/SVR}&\texttt{SPL/DCT}&\texttt{DT/SVR}&\texttt{LR/DCT}&\texttt{GP/SVR}&\texttt{DT/DCT}&\texttt{GP/SVR}&\texttt{SPL/DCT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/HIP}&\texttt{SVR/GP}&\texttt{DCT/DT}&\texttt{GP/SVR}&\texttt{SPL/DCT}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{Spark}&\texttt{DaL/DeP}&\texttt{DeP/RF}&\texttt{DT/LR}&\texttt{LR/RF}&\texttt{RF/GP}&\texttt{GP/DaL}&\texttt{RF/SPL}&\texttt{SPL/DT}&\texttt{RF/GP}&\texttt{GP/RF}&\texttt{DaL/SPL}&\texttt{SPL/RF}&\texttt{RF/GP}&\texttt{GP/RF}&\texttt{DaL/SPL}&\texttt{SPL/RF}\\
\textsc{HIPAcc}&\texttt{SVR/RF}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{RF/SVR}&\texttt{SVR/DaL}&\texttt{DeP/SVR}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{SPL/RF}&\texttt{DeP/LR}\\
\textsc{Redis}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{DaL/GP}&\texttt{GP/DeP}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/LR}&\texttt{LR/SVR}&\texttt{HIP/RF}&\texttt{RF/SVR}&\texttt{SVR/LR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{DT/GP}&\texttt{GP/SVR}&\texttt{GP/SPL}&\texttt{SPL/SVR}\\
\textsc{storm}&\texttt{LR/RF}&\texttt{SVR/DT}&\texttt{GP/RF}&\texttt{RF/DT}&\texttt{DaL/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/LR}&\texttt{DaL/DT}&\texttt{LR/RF}&\texttt{SVR/DT}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{SVR/DCT}&\texttt{DeP/RF}&\texttt{SVR/DT}&\texttt{DeP/RF}&\texttt{SPL/DT}\\
\textsc{SaC}&\texttt{DCT/HIP}&\texttt{DaL/DeP}&\texttt{DaL/RF}&\texttt{SPL/SVR}&\texttt{DaL/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/DCT}&\texttt{RF/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{RF/DeP}&\texttt{SVR/SPL}&\cellcolor{steel!30}\texttt{DCT/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{SPL/LR}\\
\textsc{Hadoop}&\texttt{SVR/SPL}&\texttt{SPL/RF}&\texttt{DT/SPL}&\texttt{SPL/RF}&\texttt{GP/DeP}&\texttt{DeP/DaL}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/DeP}&\texttt{DeP/RF}&\texttt{LR/SVR}&\texttt{SVR/RF}&\texttt{SPL/SVR}&\texttt{SVR/RF}&\texttt{HIP/SPL}&\texttt{SPL/RF}\\
\textsc{Tomcat}&\texttt{RF/DaL}&\texttt{DaL/GP}&\texttt{DT/DaL}&\texttt{DaL/RF}&\texttt{DT/DeP}&\texttt{DeP/DaL}&\texttt{DT/SVR}&\texttt{SVR/RF}&\texttt{GP/HIP}&\texttt{HIP/RF}&\texttt{RF/LR}&\texttt{LR/RF}&\texttt{DEC/GP}&\texttt{GP/RF}&\texttt{DaL/LR}&\texttt{LR/RF}\\
\textsc{JavaGC}&\texttt{SPL/RF}&\texttt{DT/SVR}&\texttt{DeP/RF}&\texttt{GP/HIP}&\texttt{DCT/HIP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{GP/SVR}&\texttt{LR/RF}&\texttt{SVR/GP}&\texttt{HIP/RF}&\texttt{SVR/HIP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/HIP}&\texttt{LR/RF}&\texttt{GP/LR}\\

%37 34 158 155
%0 4 36 40
%37 38 194 195


\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lcc|cc|cc|cc|cc|cc|cc|cc}

\multicolumn{17}{c}{}\\

\multicolumn{17}{c}{\textbf{(b) µRD and Performance}}\\

\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BOCA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ATConf}}}&\multicolumn{2}{c|}{\textbf{\texttt{FLASH}}}&\multicolumn{2}{c|}{\textbf{\texttt{OtterTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ResTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ROBOTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{SMAC}}}&\multicolumn{2}{c}{\textbf{\texttt{Tuneful}}}\\


&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}&\textbf{Best}&\textbf{Worst}\\

\midrule

%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\
\textsc{Brotli}&\texttt{DT/RF}&\texttt{DaL/DeP}&\texttt{GP/DaL}&\texttt{RF/DeP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/DCT}&\texttt{DCT/DaL}&\texttt{LR/SVR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{SVR/DeP}\\
\textsc{LLVM}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{GP/LR}&\texttt{RF/GP}&\texttt{DT/LR}&\texttt{DT/DCT}&\texttt{DaL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/SPL}&\texttt{DCT/GP}&\texttt{DaL/HIP}&\texttt{SVR/GP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{HIP/LR}&\texttt{SVR/GP}\\
\textsc{Lrzip}&\texttt{HIP/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DT/LR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/HIP}&\texttt{SVR/DCT}&\texttt{DCT/DeP}&\texttt{SPL/GP}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/SVR}&\texttt{LR/SPL}\\
\textsc{xgboost}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{GP/LR}&\texttt{DCT/GP}&\texttt{DeP/HIP}&\texttt{GP/SVR}&\texttt{DeP/HIP}&\texttt{SPL/SVR}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/LR}&\texttt{LR/GP}&\texttt{DT/RF}&\texttt{GP/SVR}&\texttt{DeP/HIP}&\texttt{LR/GP}\\
\textsc{noc-CM-log}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DaL/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{RF/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{DaL/GP}&\texttt{DeP/RF}&\texttt{SPL/GP}&\texttt{DeP/RF}&\texttt{SVR/GP}&\texttt{DeP/DT}&\texttt{DaL/GP}&\texttt{HIP/RF}&\texttt{SVR/GP}\\
\textsc{DeepArch}&\texttt{DeP/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{HIP/LR}&\texttt{SPL/GP}&\texttt{DeP/HIP}&\texttt{SPL/SVR}&\texttt{RF/HIP}&\texttt{GP/SVR}&\texttt{RF/SPL}&\texttt{DT/DeP}&\texttt{HIP/LR}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DaL/SVR}&\texttt{DaL/RF}&\texttt{SVR/GP}\\
\textsc{BDBC}&\texttt{LR/RF}&\texttt{RF/GP}&\texttt{GP/RF}&\texttt{RF/SVR}&\texttt{DeP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DeP/DT}&\texttt{SVR/GP}&\texttt{GP/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{DaL/GP}&\texttt{HIP/RF}&\texttt{SVR/GP}\\
\textsc{HSQLDB}&\texttt{SPL/DT}&\texttt{DCT/SVR}&\texttt{GP/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DT}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}\\
\textsc{DConvert}&\texttt{GP/RF}&\texttt{DeP/SVR}&\texttt{GP/RF}&\texttt{SVR/HIP}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DeP}&\texttt{DT/GP}&\texttt{HIP/DeP}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{7z}&\texttt{HIP/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{RF/DeP}&\texttt{DeP/HIP}&\texttt{SPL/SVR}&\texttt{DeP/DT}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\texttt{DCT/RF}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{GP/DeP}\\
\textsc{Apache}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DT/SPL}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{GP/SVR}&\texttt{HIP/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/DeP}&\texttt{SVR/DEC}&\texttt{DT/DaL}&\texttt{SPL/GP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{DaL/DeP}&\texttt{SVR/DEC}\\
\textsc{HSMGP}&\texttt{LR/HIP}&\texttt{GP/SVR}&\texttt{GP/HIP}&\texttt{RF/DeP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{GP/HIP}&\texttt{DCT/DeP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/DeP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{GP/SVR}&\texttt{GP/HIP}&\texttt{DCT/DeP}\\
\textsc{MongoDB}&\cellcolor{steel!30}\texttt{SPL/SPL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{RF/LR}&\texttt{SVR/DeP}&\texttt{SPL/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/SPL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DaL/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{HIP/RF}&\texttt{SVR/DeP}&\texttt{RF/LR}&\cellcolor{steel!30}\texttt{SVR/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{PostgreSQL}&\texttt{SVR/SPL}&\texttt{GP/SVR}&\texttt{DaL/SPL}&\texttt{SVR/DeP}&\texttt{DeP/DaL}&\texttt{SPL/SVR}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/DT}&\texttt{SVR/DeP}&\texttt{DaL/HIP}&\texttt{SPL/DeP}&\texttt{DCT/SPL}&\texttt{GP/SVR}&\texttt{RF/DT}&\texttt{SVR/DeP}\\
\textsc{ExaStencils}&\texttt{DeP/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}&\texttt{DeP/DaL}&\texttt{GP/LR}&\texttt{DeP/DaL}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{LR/DeP}&\texttt{GP/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SPL/DeP}\\
\textsc{kanzi}&\texttt{SPL/DeP}&\texttt{RF/GP}&\texttt{SVR/SPL}&\texttt{RF/DeP}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/HIP}&\texttt{DCT/DeP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/DeP}&\texttt{HIP/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/RF}&\texttt{RF/DeP}\\
\textsc{jump3r}&\texttt{GP/DaL}&\texttt{RF/DeP}&\texttt{GP/RF}&\texttt{SVR/DeP}&\texttt{DeP/HIP}&\texttt{SVR/DCT}&\texttt{DT/DaL}&\texttt{DeP/SPL}&\texttt{GP/LR}&\texttt{RF/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{DCT/DeP}&\texttt{SPL/RF}&\texttt{DT/GP}\\
\textsc{MariaDB}&\texttt{SPL/RF}&\texttt{DaL/DeP}&\texttt{GP/RF}&\texttt{RF/SVR}&\texttt{SPL/DaL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DCT/DT}&\texttt{SVR/DeP}&\texttt{LR/RF}&\texttt{SVR/GP}&\texttt{DeP/RF}&\texttt{SPL/GP}&\texttt{DCT/RF}&\texttt{GP/DeP}&\texttt{DT/RF}&\texttt{SPL/GP}\\
\textsc{polly}&\texttt{DCT/RF}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/GP}&\texttt{DCT/DaL}&\texttt{GP/LR}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/LR}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/HIP}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{DaL/HIP}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{SQL}&\texttt{SVR/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DeP/RF}&\texttt{SVR/DCT}&\texttt{SPL/DT}&\texttt{SVR/DeP}&\texttt{LR/DCT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{RF/SVR}&\texttt{GP/DCT}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{SVR/DCT}&\texttt{SPL/RF}&\texttt{SVR/GP}&\texttt{RF/SVR}&\texttt{GP/DCT}\\
\textsc{vp9}&\texttt{RF/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/DT}&\texttt{DT/DeP}&\texttt{LR/DT}&\texttt{GP/SVR}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{RF/DT}&\texttt{SVR/GP}&\texttt{DCT/DT}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/DT}&\cellcolor{steel!30}\texttt{GP/GP}\\
\textsc{Spark}&\texttt{DaL/SPL}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DT/RF}&\texttt{LR/DeP}&\texttt{RF/DaL}&\texttt{GP/SVR}&\texttt{RF/DaL}&\texttt{SPL/SVR}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\texttt{DaL/RF}&\texttt{SPL/DeP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/DeP}&\texttt{DaL/RF}&\texttt{SPL/DeP}\\
\textsc{HIPAcc}&\texttt{SVR/SPL}&\texttt{GP/SVR}&\texttt{GP/RF}&\texttt{RF/DeP}&\texttt{SVR/DaL}&\texttt{DeP/SVR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{DaL/RF}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{SPL/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}\\
\textsc{Redis}&\texttt{SVR/HIP}&\texttt{GP/DeP}&\texttt{DaL/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{SPL/RF}&\texttt{SVR/GP}&\texttt{HIP/DT}&\texttt{LR/GP}&\texttt{HIP/SVR}&\texttt{RF/DeP}&\texttt{SVR/RF}&\texttt{LR/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{GP/GP}&\texttt{GP/DEC}&\texttt{SPL/DeP}\\
\textsc{storm}&\texttt{LR/DT}&\texttt{SVR/DeP}&\texttt{GP/RF}&\texttt{RF/SVR}&\cellcolor{steel!30}\texttt{DaL/DaL}&\texttt{RF/DeP}&\texttt{GP/DaL}&\texttt{DaL/DeP}&\texttt{LR/RF}&\cellcolor{steel!30}\texttt{SVR/SVR}&\texttt{LR/RF}&\texttt{SVR/GP}&\texttt{DeP/DT}&\texttt{SVR/DeP}&\texttt{DeP/DT}&\texttt{SPL/GP}\\
\textsc{SaC}&\texttt{DCT/HIP}&\texttt{DaL/SVR}&\texttt{DaL/HIP}&\texttt{SPL/SVR}&\texttt{DaL/RF}&\texttt{DeP/SVR}&\texttt{HIP/DCT}&\texttt{RF/SVR}&\texttt{DT/SVR}&\cellcolor{steel!30}\texttt{LR/LR}&\texttt{RF/DeP}&\texttt{SVR/DCT}&\texttt{DCT/DT}&\texttt{DeP/SVR}&\texttt{DeP/SVR}&\texttt{SPL/LR}\\
\textsc{Hadoop}&\texttt{SVR/RF}&\texttt{SPL/DeP}&\texttt{DT/RF}&\texttt{SPL/DeP}&\texttt{GP/DT}&\cellcolor{steel!30}\texttt{DeP/DeP}&\cellcolor{steel!30}\texttt{DT/DT}&\texttt{RF/DeP}&\texttt{DT/RF}&\cellcolor{steel!30}\texttt{DeP/DeP}&\texttt{LR/RF}&\texttt{SVR/DeP}&\texttt{SPL/RF}&\texttt{SVR/DeP}&\texttt{HIP/RF}&\texttt{SPL/DeP}\\
\textsc{Tomcat}&\texttt{RF/LR}&\texttt{DaL/SVR}&\texttt{DT/RF}&\texttt{DaL/GP}&\texttt{DT/DaL}&\texttt{DeP/SVR}&\texttt{DT/DaL}&\texttt{SVR/DeP}&\texttt{GP/RF}&\texttt{HIP/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{LR/GP}&\texttt{DEC/RF}&\texttt{GP/SVR}&\texttt{DaL/RF}&\texttt{LR/GP}\\
\textsc{JavaGC}&\cellcolor{steel!30}\texttt{SPL/SPL}&\texttt{DT/SVR}&\texttt{DeP/RF}&\texttt{GP/SVR}&\texttt{DCT/HIP}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}\texttt{DCT/DCT}&\texttt{GP/SVR}&\texttt{LR/SPL}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{HIP/HIP}&\texttt{SVR/GP}&\cellcolor{steel!30}\texttt{RF/RF}&\texttt{GP/SVR}&\texttt{LR/SVR}&\texttt{GP/LR}\\

%46 49 143 146
%5 8 32 35
%51 57 175 181

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ3/rq3_MFO_eff.tex <==
\begin{table*}[t!]
\caption{Spearman correlations between model accuracy and its resulting tuning efficiency for batch model-based tuners. The formats are the same as Table~\ref{tb:rq4_smbt_perf}.}
\label{tb:rq4_bmbt_eff}
%\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize

\begin{adjustbox}{width=\textwidth,center} %\0.88
\begin{tabular}{lc|c|c|c|c|c|c|c|c}

\multicolumn{10}{c}{\textbf{(a) MAPE and Efficiency}}\\

\toprule


\textbf{System}&\textbf{\texttt{BestConfig}}&\textbf{\texttt{Irace}}&\textbf{\texttt{GGA}}&\textbf{\texttt{ParamILS}}&\textbf{\texttt{R\_Search}}&\textbf{\texttt{GA}}&\textbf{\texttt{SWAY}}&\textbf{\texttt{ConEx}}&\textbf{\texttt{E\_search}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}. Note if negative, a  $-$ should be placed beforehand.

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&-&-&-&-&-&-&-&-&$-$\percent[n]{0.28}{1}{0.28$^\dagger$}{40}\\
\textsc{LLVM}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}\\
\textsc{Lrzip}&-&-&-&-&-&-&-&-&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\
\textsc{xgboost}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{noc-CM-log}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}\\
\textsc{DeepArch}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}\\
\textsc{BDBC}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}\\
\textsc{HSQLDB}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}\\
\textsc{DConvert}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&-\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.76}{1}{0.76$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&-\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&-\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&-\\
\textsc{MongoDB}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&-\\
\textsc{PostgreSQL}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&-\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.57}{1}{0.57$^\dagger$}{60}&-\\
\textsc{kanzi}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&-\\
\textsc{jump3r}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&-\\
\textsc{MariaDB}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&-\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&-\\
\textsc{SQL}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&-\\
\textsc{vp9}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&-\\
\textsc{Spark}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&-\\
\textsc{HIPAcc}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.76}{1}{0.76$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&-\\
\textsc{Redis}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&-\\
\textsc{storm}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&-\\
\textsc{SaC}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&-\\
\textsc{Hadoop}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&-\\
\textsc{Tomcat}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}&-\\
\textsc{JavaGC}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&-\\





\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lc|c|c|c|c|c|c|c|c}

\multicolumn{10}{c}{}\\

\multicolumn{10}{c}{\textbf{(b) µRD and Efficiency}}\\

\toprule

\textbf{System}&\textbf{\texttt{BestConfig}}&\textbf{\texttt{Irace}}&\textbf{\texttt{GGA}}&\textbf{\texttt{ParamILS}}&\textbf{\texttt{R\_Search}}&\textbf{\texttt{GA}}&\textbf{\texttt{SWAY}}&\textbf{\texttt{ConEx}}&\textbf{\texttt{E\_search}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&-&-&-&-&-&-&-&-&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}\\
\textsc{LLVM}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}\\
\textsc{Lrzip}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}\\
\textsc{xgboost}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{noc-CM-log}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}\\
\textsc{DeepArch}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}\\
\textsc{BDBC}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}\\
\textsc{HSQLDB}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}\\
\textsc{DConvert}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.55}{1}{0.55$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&-\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&-\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&-\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&-\\
\textsc{MongoDB}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&-\\
\textsc{PostgreSQL}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&-\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.56}{1}{0.56$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.57}{1}{0.57$^\dagger$}{60}&-\\
\textsc{kanzi}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&-\\
\textsc{jump3r}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&-\\
\textsc{MariaDB}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&-\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&-\\
\textsc{SQL}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}&-\\
\textsc{vp9}&$-$\percent[n]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&-\\
\textsc{Spark}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&-\\
\textsc{HIPAcc}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.74}{1}{0.74$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&-\\
\textsc{Redis}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&-\\
\textsc{storm}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&-\\
\textsc{SaC}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}&-\\
\textsc{Hadoop}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&-\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&-\\
\textsc{JavaGC}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.74}{1}{0.74$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&-\\




\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ3/rq3_MFO_perf.tex <==
\begin{table*}[t!]
\caption{Spearman correlations between model accuracy and its resulting tuning performance for batch model-based tuners. The formats are the same as Table~\ref{tb:rq4_smbt_perf}.}
\label{tb:rq4_bmbt_eff}
%\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center} %\0.88
\begin{tabular}{lc|c|c|c|c|c|c|c|c}

\multicolumn{10}{c}{\textbf{(a) MAPE and Performance}}\\

\toprule


\textbf{System}&\textbf{\texttt{BestConfig}}&\textbf{\texttt{Irace}}&\textbf{\texttt{GGA}}&\textbf{\texttt{ParamILS}}&\textbf{\texttt{R\_Search}}&\textbf{\texttt{GA}}&\textbf{\texttt{SWAY}}&\textbf{\texttt{ConEx}}&\textbf{\texttt{E\_search}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}. Note if negative, a  $-$ should be placed beforehand.

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}\\
\textsc{LLVM}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}\\
\textsc{Lrzip}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{xgboost}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{noc-CM-log}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}\\
\textsc{DeepArch}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}\\
\textsc{BDBC}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}\\
\textsc{HSQLDB}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}\\
\textsc{DConvert}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&-\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.72}{1}{0.72$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.79}{1}{0.79$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.76}{1}{0.76$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.79}{1}{0.79$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&-\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&-\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&-\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.56}{1}{0.56$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.55}{1}{0.55$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&-\\
\textsc{PostgreSQL}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&-\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.67}{1}{0.67$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.63}{1}{0.63$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.65}{1}{0.65$^\dagger$}{60}&-\\
\textsc{kanzi}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&-\\
\textsc{jump3r}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&-\\
\textsc{MariaDB}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&-\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&-\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&-\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&-\\
\textsc{Spark}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&-\\
\textsc{HIPAcc}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.62}{1}{0.62$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.65}{1}{0.65$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.73}{1}{0.73$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.67}{1}{0.67$^\dagger$}{60}&-\\
\textsc{Redis}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{storm}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&-\\
\textsc{SaC}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.55}{1}{0.55$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.70}{1}{0.70$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&-\\
\textsc{Hadoop}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&-\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&-\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.73}{1}{0.73$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.67}{1}{0.67$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.67}{1}{0.67$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&-\\





\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lc|c|c|c|c|c|c|c|c}

\multicolumn{10}{c}{}\\

\multicolumn{10}{c}{\textbf{(b) µRD and Performance}}\\

\toprule

\textbf{System}&\textbf{\texttt{BestConfig}}&\textbf{\texttt{Irace}}&\textbf{\texttt{GGA}}&\textbf{\texttt{ParamILS}}&\textbf{\texttt{R\_Search}}&\textbf{\texttt{GA}}&\textbf{\texttt{SWAY}}&\textbf{\texttt{ConEx}}&\textbf{\texttt{E\_search}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}\\
\textsc{LLVM}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}\\
\textsc{Lrzip}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}\\
\textsc{xgboost}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}\\
\textsc{noc-CM-log}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}\\
\textsc{DeepArch}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}\\
\textsc{BDBC}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.55}{1}{0.55$^\dagger$}{60}\\
\textsc{HSQLDB}&-&-&-&-&-&-&-&-&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}\\
\textsc{DConvert}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&-\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.69}{1}{0.69$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.77}{1}{0.77$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.77}{1}{0.77$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.80}{1}{0.80$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&-\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&-\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&-\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.54}{1}{0.54$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.56}{1}{0.56$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.57}{1}{0.57$^\dagger$}{60}&-\\
\textsc{PostgreSQL}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&-\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.63}{1}{0.63$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.65}{1}{0.65$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.63}{1}{0.63$^\dagger$}{60}&-\\
\textsc{kanzi}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&-\\
\textsc{jump3r}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.62}{1}{0.62$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.63}{1}{0.63$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.72}{1}{0.72$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.69}{1}{0.69$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&-\\
\textsc{MariaDB}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.56}{1}{0.56$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&-\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&-\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&-\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&-\\
\textsc{Spark}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.56}{1}{0.56$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&-\\
\textsc{HIPAcc}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.68}{1}{0.68$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.65}{1}{0.65$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.74}{1}{0.74$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.69}{1}{0.69$^\dagger$}{60}&-\\
\textsc{Redis}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&-\\
\textsc{storm}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.57}{1}{0.57$^\dagger$}{60}&-\\
\textsc{SaC}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.55}{1}{0.55$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.62}{1}{0.62$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.61}{1}{0.61$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&-\\
\textsc{Hadoop}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&-\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.61}{1}{0.61$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&-\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.76}{1}{0.76$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.80}{1}{0.80$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.78}{1}{0.78$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.75}{1}{0.75$^\dagger$}{80}&-\\





\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ3/rq3_SMBO_eff.tex <==
\begin{table*}[t!]
\caption{Spearman correlations between model accuracy and its resulting tuning efficiency for sequential model-based tuners. The formats are the same as Table~\ref{tb:rq4_smbt_perf}.}
\label{tb:rq4_smbt_eff}
%\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center} %\0.88
\begin{tabular}{lc|c|c|c|c|c|c|c}

\multicolumn{9}{c}{\textbf{(a) MAPE and Efficiency}}\\

\toprule


\textbf{System}&\textbf{\texttt{BOCA}}&\textbf{\texttt{ATConf}}&\textbf{\texttt{FLASH}}&\textbf{\texttt{OtterTune}}&\textbf{\texttt{ResTune}}&\textbf{\texttt{ROBOTune}}&\textbf{\texttt{SMAC}}&\textbf{\texttt{Tuneful}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}. Note if negative, a  $-$ should be placed beforehand.

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&$-$\percent[n]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\
\textsc{LLVM}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{Lrzip}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{xgboost}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}\\
\textsc{noc-CM-log}&$-$\percent[n]{0.32}{1}{0.32$^\dagger$}{40}&$-$\percent[n]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.69}{1}{0.69$^\dagger$}{60}&$-$\percent[n]{0.49}{1}{0.49$^\dagger$}{60}&$-$\percent[n]{0.30}{1}{0.30$^\dagger$}{40}\\
\textsc{DeepArch}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{BDBC}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.35}{1}{0.35$^\dagger$}{40}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.32}{1}{0.32$^\dagger$}{40}&$-$\percent[n]{0.37}{1}{0.37$^\dagger$}{40}\\
\textsc{HSQLDB}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}&$-$\percent[n]{0.41}{1}{0.41$^\dagger$}{60}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}\\
\textsc{DConvert}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{7z}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.48}{1}{0.48$^\dagger$}{60}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}\\
\textsc{HSMGP}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.33}{1}{0.33$^\dagger$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{PostgreSQL}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}\\
\textsc{kanzi}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}\\
\textsc{jump3r}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&$-$\percent[n]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}\\
\textsc{MariaDB}&$-$\percent[n]{0.25}{1}{0.25$^\dagger$}{40}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.30}{1}{0.30$^\dagger$}{40}&$-$\percent[n]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{Spark}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.19}{1}{0.19$^\dagger$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{HIPAcc}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\
\textsc{Redis}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}\\
\textsc{storm}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{SaC}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}\\
\textsc{Hadoop}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\




\bottomrule
\end{tabular}

\end{adjustbox}


\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lc|c|c|c|c|c|c|c}

\multicolumn{9}{c}{}\\

\multicolumn{9}{c}{\textbf{(b) µRD and Efficiency}}\\

\toprule


\textbf{System}&\textbf{\texttt{BOCA}}&\textbf{\texttt{ATConf}}&\textbf{\texttt{FLASH}}&\textbf{\texttt{OtterTune}}&\textbf{\texttt{ResTune}}&\textbf{\texttt{ROBOTune}}&\textbf{\texttt{SMAC}}&\textbf{\texttt{Tuneful}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{LLVM}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{Lrzip}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{xgboost}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{noc-CM-log}&$-$\percent[n]{0.28}{1}{0.28$^\dagger$}{40}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.58}{1}{0.58$^\dagger$}{60}&$-$\percent[n]{0.50}{1}{0.50$^\dagger$}{60}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}\\
\textsc{DeepArch}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}\\
\textsc{BDBC}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.22}{1}{0.22$^\dagger$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.39}{1}{0.39$^\dagger$}{60}&$-$\percent[n]{0.42}{1}{0.42$^\dagger$}{60}\\
\textsc{HSQLDB}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{DConvert}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{7z}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{PostgreSQL}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.40}{1}{0.40$^\dagger$}{60}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}\\
\textsc{kanzi}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}\\
\textsc{jump3r}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{MariaDB}&$-$\percent[n]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&$-$\percent[n]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}\\
\textsc{Spark}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{HIPAcc}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{Redis}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}\\
\textsc{storm}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.30}{1}{0.30$^\dagger$}{40}&$-$\percent[n]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{SaC}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{Hadoop}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\







\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> Tables/RQ3/rq3_SMBO_perf.tex <==
\begin{table*}[t!]
\caption{Spearman correlations between model accuracy and its resulting tuning performance for sequential model-based tuners. $^\dagger$ and $^\star$ denote $p<0.001$ and $0.001 \leq p<0.05$, respectively. \colorbox{steel!30}{Blue bars} and \colorbox{red!30}{red bars} indicate positive and negative correlation, respectively. The number and bar length show strength.}
\label{tb:rq4_smbt_perf}

\centering
\begin{minipage}{.49\textwidth}
\setlength{\tabcolsep}{0.7mm}
\centering
\footnotesize
\subfloat[MAPE and performance]{
\begin{adjustbox}{width=\textwidth,center} %\0.88

\begin{tabular}{lc|c|c|c|c|c|c|c}

%\multicolumn{9}{c}{\textbf{(a) MAPE and Performance}}\\

\toprule


\textbf{System}&\textbf{\texttt{BOCA}}&\textbf{\texttt{ATConf}}&\textbf{\texttt{FLASH}}&\textbf{\texttt{OtterTune}}&\textbf{\texttt{ResTune}}&\textbf{\texttt{ROBOTune}}&\textbf{\texttt{SMAC}}&\textbf{\texttt{Tuneful}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}. Note if negative, a  $-$ should be placed beforehand.

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&$-$\percent[n]{0.53}{1}{0.53$^\dagger$}{60}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{LLVM}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{100}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.74}{1}{0.74$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{Lrzip}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}\\
\textsc{xgboost}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.57}{1}{0.57$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}\\
\textsc{noc-CM-log}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&$-$\percent[n]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}\\
\textsc{DeepArch}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{BDBC}&$-$\percent[n]{0.21}{1}{0.21$^\dagger$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&$-$\percent[n]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}\\
\textsc{HSQLDB}&$-$\percent[n]{0.26}{1}{0.26$^\dagger$}{40}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.62}{1}{0.62$^\dagger$}{60}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{DConvert}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.54}{1}{0.54$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.63}{1}{0.63$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.59}{1}{0.59$^\dagger$}{60}&$-$\percent[n]{0.51}{1}{0.51$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.59}{1}{0.59$^\dagger$}{60}\\
\textsc{HSMGP}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.50}{1}{0.50$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.60}{1}{0.60$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}\\
\textsc{PostgreSQL}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&$-$\percent[n]{0.27}{1}{0.27$^\dagger$}{40}&$-$\percent[n]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.59}{1}{0.59$^\dagger$}{60}&$-$\percent[n]{0.16}{1}{0.16$^\star$}{40}\\
\textsc{kanzi}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&$-$\percent[n]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}\\
\textsc{jump3r}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&$-$\percent[n]{0.45}{1}{0.45$^\dagger$}{60}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}\\
\textsc{MariaDB}&$-$\percent[n]{0.37}{1}{0.37$^\dagger$}{40}&$-$\percent[n]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.36}{1}{0.36$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}\\
\textsc{Spark}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{HIPAcc}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{Redis}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{storm}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{100}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{SaC}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{Hadoop}&$-$\percent[n]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.54}{1}{0.54$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}\\




\bottomrule
\end{tabular}


\end{adjustbox}
}
\end{minipage}
\begin{minipage}{.49\textwidth}

\setlength{\tabcolsep}{0.7mm}
\centering
\footnotesize
\subfloat[$\mu$RD and performance]{
\begin{adjustbox}{width=\textwidth,center}

\begin{tabular}{lc|c|c|c|c|c|c|c}

%\multicolumn{9}{c}{}\\

%\multicolumn{9}{c}{\textbf{(b) $\mu$RD and Performance}}\\

\toprule


\textbf{System}&\textbf{\texttt{BOCA}}&\textbf{\texttt{ATConf}}&\textbf{\texttt{FLASH}}&\textbf{\texttt{OtterTune}}&\textbf{\texttt{ResTune}}&\textbf{\texttt{ROBOTune}}&\textbf{\texttt{SMAC}}&\textbf{\texttt{Tuneful}}\\


\midrule

%\percent[p is positive, n is negative]{r value}{1}{r value + the symbol for representing p result}{the color classification}

%$0 \leq |r| \leq 0.09$ is negligible; $0.09 < |r| \leq 0.39$ implies weak; $0.39 < |r| \leq 0.69$ is considered as moderate; $0.69 < |r| \leq 0.89$ is strong, and $0.89 < |r| \leq 1$ means very strong.

%the color classification = 20 negligible; 40 weak; 60 moderate; 80 strong; 100 very strong.

\textsc{Brotli}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{60}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{LLVM}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{100}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.71}{1}{0.71$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}\\
\textsc{Lrzip}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&$-$\percent[n]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.14}{1}{0.14$^\star$}{40}\\
\textsc{xgboost}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}\\
\textsc{noc-CM-log}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&$-$\percent[n]{0.14}{1}{0.14$^\star$}{40}&$-$\percent[n]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.42}{1}{0.42$^\dagger$}{60}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{DeepArch}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}\\
\textsc{BDBC}&$-$\percent[n]{0.22}{1}{0.22$^\dagger$}{40}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&$-$\percent[n]{0.15}{1}{0.15$^\star$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}\\
\textsc{HSQLDB}&$-$\percent[n]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.46}{1}{0.46$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.30}{1}{0.30$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}\\
\textsc{DConvert}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.28}{1}{0.28$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.37}{1}{0.37$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.53}{1}{0.53$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{7z}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.62}{1}{0.62$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.69}{1}{0.69$^\dagger$}{80}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{Apache}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}\\
\textsc{HSMGP}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&$-$\percent[n]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.33}{1}{0.33$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}\\
\textsc{MongoDB}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.20}{1}{0.20$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.54}{1}{0.54$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.52}{1}{0.52$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.58}{1}{0.58$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.23}{1}{0.23$^\dagger$}{40}\\
\textsc{PostgreSQL}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{20}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{ExaStencils}&\phantom{$-$}\percent[p]{0.38}{1}{0.38$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.69}{1}{0.69$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.65}{1}{0.65$^\dagger$}{60}&$-$\percent[n]{0.19}{1}{0.19$^\dagger$}{40}&$-$\percent[n]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.66}{1}{0.66$^\dagger$}{60}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{kanzi}&$-$\percent[n]{0.06}{1}{0.06$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.50}{1}{0.50$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.39}{1}{0.39$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.26}{1}{0.26$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}\\
\textsc{jump3r}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.49}{1}{0.49$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}\\
\textsc{MariaDB}&$-$\percent[n]{0.36}{1}{0.36$^\dagger$}{40}&$-$\percent[n]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.51}{1}{0.51$^\dagger$}{60}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.47}{1}{0.47$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}\\
\textsc{polly}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.08}{1}{0.08$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{SQL}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.31}{1}{0.31$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.13}{1}{0.13$^\star$}{40}&\phantom{$-$}\percent[p]{0.06}{1}{0.06$^{\,\,\,}$}{20}\\
\textsc{vp9}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.41}{1}{0.41$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.43}{1}{0.43$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.45}{1}{0.45$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}\\
\textsc{Spark}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.40}{1}{0.40$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.21}{1}{0.21$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.25}{1}{0.25$^\dagger$}{40}\\
\textsc{HIPAcc}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.44}{1}{0.44$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.27}{1}{0.27$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}\\
\textsc{Redis}&$-$\percent[n]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&$-$\percent[n]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&$-$\percent[n]{0.29}{1}{0.29$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.05}{1}{0.05$^{\,\,\,}$}{20}\\
\textsc{storm}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&$-$\percent[n]{0.35}{1}{0.35$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.00}{1}{0.00$^{\,\,\,}$}{100}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\dagger$}{40}&$-$\percent[n]{0.05}{1}{0.05$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}\\
\textsc{SaC}&$-$\percent[n]{0.04}{1}{0.04$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.19}{1}{0.19$^\star$}{40}&$-$\percent[n]{0.11}{1}{0.11$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.48}{1}{0.48$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.02}{1}{0.02$^{\,\,\,}$}{20}\\
\textsc{Hadoop}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}&$-$\percent[n]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.07}{1}{0.07$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.17}{1}{0.17$^\star$}{40}&$-$\percent[n]{0.12}{1}{0.12$^\star$}{40}&$-$\percent[n]{0.18}{1}{0.18$^\star$}{40}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.04}{1}{0.04$^{\,\,\,}$}{20}\\
\textsc{Tomcat}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{40}&\phantom{$-$}\percent[p]{0.12}{1}{0.12$^\star$}{40}&\phantom{$-$}\percent[p]{0.34}{1}{0.34$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.24}{1}{0.24$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.03}{1}{0.03$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.09}{1}{0.09$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.10}{1}{0.10$^{\,\,\,}$}{40}&$-$\percent[n]{0.11}{1}{0.11$^\star$}{40}\\
\textsc{JavaGC}&\phantom{$-$}\percent[p]{0.16}{1}{0.16$^\star$}{40}&$-$\percent[n]{0.02}{1}{0.02$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&\phantom{$-$}\percent[p]{0.64}{1}{0.64$^\dagger$}{60}&$-$\percent[n]{0.01}{1}{0.01$^{\,\,\,}$}{20}&\phantom{$-$}\percent[p]{0.22}{1}{0.22$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.32}{1}{0.32$^\dagger$}{40}&\phantom{$-$}\percent[p]{0.01}{1}{0.01$^{\,\,\,}$}{20}\\







\bottomrule
\end{tabular}

\end{adjustbox}
}
\end{minipage}

\end{table*}

==> Tables/RQ3_MAPE.tex <==
\begin{table}[t!]
\centering
\footnotesize
\caption{A Summary of RQ4 MAPE results}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lllp{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
\toprule

\textbf{Optimization}&\textbf{Target}  &\textbf{Trend} & \textbf{0\%}& \textbf{10\%} & \textbf{20\%} & \textbf{30\%}& \textbf{40\%}& \textbf{50\%}& \textbf{60\%}& \textbf{70\%}& \textbf{80\%}& \textbf{90\%}& \textbf{\textgreater100\%}  \\ 
\midrule

MFO& PERF. & Improve &1.01\%&7.85\%&12.49\%&22.23\%&32.39\%&26.16\%&42.45\%&56.01\%&59.51\%&70.17\%&70.37\% \\
\rowcolor{steel!10}MFO&PERF. & Lower &0.77\%&6.1\%&8.05\%&17.3\%&21.04\%&5.19\%& - &60.77\%&5.43\%&35.03\%&49.81\% \\
MFO&EFF. & Improve &1.16\%&8.95\%&12.94\%&22.34\%&28.48\%&28.97\%&42.64\%&61.47\%&65.07\%&67.07\%&83.18\% \\
\rowcolor{steel!10}MFO&EFF. & Lower &1.47\%&7.9\%&11.2\%&13.71\%&20.52\%&27.35\%&30.76\%&12.58\%&49.35\%&36.81\%&71.78\% \\

SMBO& PERF. & Improve &1.02\%&4.57\%&6.13\%&13.0\%&23.47\%&21.4\%&23.35\%&30.65\%&27.63\%&35.12\%&67.67\% \\
\rowcolor{steel!10}SMBO&PERF & Lower &0.74\%&2.85\%&4.35\%&8.19\%&9.2\%&20.3\%&23.17\%&25.27\%&15.34\%&27.35\%&58.23\% \\
SMBO&EFF. & Improve &0.94\%&5.42\%&7.28\%&12.18\%&17.55\%&20.02\%&27.31\%&30.69\%&30.18\%&41.25\%&54.69\% \\
\rowcolor{steel!10}SMBO&EFF  & Lower &0.95\%&3.39\%&5.71\%&9.09\%&15.85\%&20.12\%&24.94\%&30.4\%&28.29\%&27.86\%&52.87\% \\


\bottomrule

\end{tabular}
\end{adjustbox}
\label{tb:rq4_MAPE}
\end{table}

==> Tables/RQ3_rank.tex <==
\begin{table}[t!]
\centering
\footnotesize
\caption{A Summary of RQ4 µRD results}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lllp{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}}
\toprule


\textbf{Optimization} & \textbf{Target} & \textbf{Trend} & \textbf{0\%} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%} & \textbf{40\%} & \textbf{50\%} & \textbf{60\%} & \textbf{70\%} & \textbf{80\%} & \textbf{90\%} & \textbf{\textgreater100\%} \\
\midrule

MFO & PERF. & Improve & 0.98\% & 4.52\% & 9.47\% & 15.24\% & - & - & - & - & - & - & - \\
\rowcolor{steel!10}MFO & PERF. & Lower & 0.79\% & 3.17\% & 4.4\% & 13.47\% & - & - & - & - & - & - & - \\
MFO & EFF. & Improve & 1.39\% & 5.13\% & 11.01\% & 18.45\% & - & - & - & - & - & - & - \\
\rowcolor{steel!10}MFO & EFF. & Lower & 0.8\% & 4.39\% & 8.26\% & 14.44\% & - & - & - & - & - & - & - \\

SMBO & PERF. & Improve & 0.76\% & 1.87\% & 4.52\% & 10.42\% & 26.97\% & - & - & - & - & - & - \\
\rowcolor{steel!10}SMBO & PERF. & Lower & 0.74\% & 1.11\% & 1.43\% & 3.97\% & 7.59\% & 31.41\% & - & - & - & - & - \\
SMBO & EFF. & Improve & 1.03\% & 1.83\% & 4.54\% & 10.52\% & 25.62\% & - & - & - & - & - & - \\
\rowcolor{steel!10}SMBO & EFF. & Lower & 1.11\% & 1.52\% & 4.4\% & 7.34\% & 38.43\% & - & - & - & - & - & - \\




\bottomrule

\end{tabular}
\end{adjustbox}
\label{tb:rq4_rank}
\end{table}

==> Tables/RQ5/SMBO_eff-old.tex <==
\begin{table*}[t!]
\caption{The results difference of original model and best substitute model of PERF. in SMBO (DaL/DaL means the first is based on performance while the latter is based on original SMBO). Only round to 2 decimal places for Impr.. Abbreviation restricted to at most 3 words for model: DeepPerf-DeP, HINNPerf-HIP, SPLConquer-SPL, DECART-DCT. Use $^\dagger$ for $p<0.001$; Use $^\star$ for $0.001 \leq p<0.05$; Otherwise using $^{\,\,\,}$. Systems use textsc while models/optimizers use texttt effect.}
\label{tb:rq5_eff}
\setlength{\tabcolsep}{0.5mm}
\centering
\footnotesize
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{lll|ll|ll|ll|ll|ll|ll|ll}


\toprule


\multirow{2}{*}{\textbf{System}}&\multicolumn{2}{c|}{\textbf{\texttt{BOCA}}}&\multicolumn{2}{c|}{\textbf{\texttt{ATConf}}}&\multicolumn{2}{c|}{\textbf{\texttt{FLASH}}}&\multicolumn{2}{c|}{\textbf{\texttt{OtterTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ResTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{ROBOTune}}}&\multicolumn{2}{c|}{\textbf{\texttt{SMAC}}}&\multicolumn{2}{c}{\textbf{\texttt{Tuneful}}}\\


&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}&\textbf{Model}&\textbf{Impr.}\\

\midrule


%\textsc{Trimesh}&$\{$Latency (s), \# Iterations$\}$&$\{81,4\}$&$\{461,15\}$&$\{135,7\}$&$\{37,501\}$\\




\textsc{Brotli}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{212.84\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{54.20\%$^\star$}&\cellcolor{red!30}\texttt{LR/DT}&\cellcolor{red!30}{119.01\%$^\dagger$}&\texttt{SVR/GP}&{10.68\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{85.16\%$^\star$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{285.96\%$^\dagger$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{103.42\%$^\dagger$}&\texttt{SPL/GP}&{61.48\%$^{\,\,\,}$}\\
\textsc{LLVM}&\cellcolor{red!30}\texttt{HIP/RF}&\cellcolor{red!30}{99.47\%$^\dagger$}&\texttt{SPL/GP}&{34.51\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SPL/DT}&\cellcolor{red!30}{49.54\%$^\star$}&\texttt{LR/GP}&{36.24\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SPL/GP}&{74.43\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{246.67\%$^\dagger$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{Lrzip}&\texttt{DaL/RF}&{16.89\%$^{\,\,\,}$}&\texttt{RF/GP}&{11.02\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SVR/DT}&\cellcolor{red!30}{121.95\%$^\dagger$}&\texttt{SVR/GP}&{39.67\%$^{\,\,\,}$}&\texttt{SVR/GP}&{5.12\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{96.97\%$^\dagger$}&\texttt{HIP/GP}&{15.04\%$^{\,\,\,}$}\\
\textsc{xgboost}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SPL/GP}&{20.64\%$^{\,\,\,}$}&\texttt{RF/DT}&{15.28\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/GP}&\cellcolor{red!30}{102.87\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/RF}&\cellcolor{red!30}{50.49\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{noc-CM-log}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{73.66\%$^\star$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{312.55\%$^\dagger$}&\cellcolor{red!30}\texttt{DeP/DT}&\cellcolor{red!30}{35.62\%$^\star$}&\cellcolor{red!30}\texttt{SVR/GP}&\cellcolor{red!30}{63.53\%$^\star$}&\cellcolor{red!30}\texttt{DeP/GP}&\cellcolor{red!30}{199.54\%$^\dagger$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{78.53\%$^\star$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{178.28\%$^\dagger$}&\cellcolor{red!30}\texttt{HIP/GP}&\cellcolor{red!30}{177.50\%$^\dagger$}\\
\textsc{DeepArch}&\texttt{DeP/RF}&{7.07\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{RF/DT}&{41.85\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{HIP/GP}&\cellcolor{red!30}{91.55\%$^\dagger$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{LR/GP}&{3.75\%$^{\,\,\,}$}\\
\textsc{BDBC}&\texttt{DeP/RF}&{52.23\%$^{\,\,\,}$}&\texttt{LR/GP}&{4.87\%$^{\,\,\,}$}&\texttt{RF/DT}&{15.87\%$^{\,\,\,}$}&\texttt{RF/GP}&{19.16\%$^{\,\,\,}$}&\texttt{LR/GP}&{6.39\%$^{\,\,\,}$}&\texttt{LR/GP}&{43.13\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{484.03\%$^\dagger$}&\texttt{LR/GP}&{62.97\%$^{\,\,\,}$}\\
\textsc{HSQLDB}&\texttt{GP/RF}&{25.37\%$^{\,\,\,}$}&\texttt{SPL/GP}&{45.80\%$^{\,\,\,}$}&\texttt{DaL/DT}&{11.98\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{RF/GP}&\cellcolor{red!30}{95.93\%$^\star$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{83.37\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{228.43\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{108.50\%$^\star$}\\
\textsc{DConvert}&\texttt{HIP/RF}&{15.76\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{HIP/DT}&{54.36\%$^{\,\,\,}$}&\texttt{DT/GP}&{47.23\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SVR/GP}&{62.70\%$^{\,\,\,}$}&\texttt{GP/RF}&{63.48\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{7z}&\texttt{DaL/RF}&{42.70\%$^{\,\,\,}$}&\texttt{DeP/GP}&{12.35\%$^{\,\,\,}$}&\texttt{DaL/DT}&{66.35\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{250.06\%$^\star$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{231.46\%$^\dagger$}&\texttt{RF/GP}&{80.69\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{224.88\%$^\dagger$}\\
\textsc{HSMGP}&\cellcolor{red!30}\texttt{HIP/RF}&\cellcolor{red!30}{284.28\%$^\star$}&\texttt{SPL/GP}&{19.79\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{HIP/DT}&\cellcolor{red!30}{264.59\%$^\dagger$}&\texttt{HIP/GP}&{69.65\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{157.18\%$^\dagger$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{326.87\%$^\star$}&\cellcolor{red!30}\texttt{SPL/RF}&\cellcolor{red!30}{281.16\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{159.57\%$^\dagger$}\\
\textsc{MongoDB}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SPL/GP}&{27.70\%$^{\,\,\,}$}&\texttt{LR/DT}&{37.96\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{235.72\%$^\dagger$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SVR/GP}&{52.02\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SPL/RF}&\cellcolor{red!30}{191.32\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{53.78\%$^\star$}\\
\textsc{PostgreSQL}&\cellcolor{red!30}\texttt{LR/RF}&\cellcolor{red!30}{75.54\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/DT}&\cellcolor{red!30}{648.50\%$^\dagger$}&\texttt{RF/GP}&{24.70\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{HIP/GP}&\cellcolor{red!30}{48.97\%$^\star$}&\texttt{DaL/GP}&{69.06\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{276.45\%$^\dagger$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{38.33\%$^\star$}\\
\textsc{ExaStencils}&\texttt{HIP/RF}&{26.14\%$^{\,\,\,}$}&\texttt{RF/GP}&{77.56\%$^{\,\,\,}$}&\texttt{DaL/DT}&{22.28\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{699.63\%$^\dagger$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{RF/GP}&{38.58\%$^{\,\,\,}$}\\
\textsc{kanzi}&\cellcolor{red!30}\texttt{LR/RF}&\cellcolor{red!30}{92.16\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{RF/DT}&{31.77\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{RF/GP}&\cellcolor{red!30}{303.58\%$^\dagger$}&\texttt{SVR/GP}&{25.45\%$^{\,\,\,}$}&\texttt{SVR/GP}&{4.98\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SPL/RF}&\cellcolor{red!30}{143.12\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{jump3r}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{116.26\%$^\star$}&\texttt{SPL/GP}&{2.76\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/DT}&\cellcolor{red!30}{59.67\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SVR/GP}&{14.90\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{HIP/RF}&\cellcolor{red!30}{184.12\%$^\star$}&\texttt{SPL/GP}&{7.27\%$^{\,\,\,}$}\\
\textsc{MariaDB}&\cellcolor{red!30}\texttt{LR/RF}&\cellcolor{red!30}{209.52\%$^\dagger$}&\texttt{SPL/GP}&{33.23\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{DT/DT}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SPL/GP}&{58.98\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{79.81\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{GP/RF}&{28.91\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{85.51\%$^\star$}\\
\textsc{polly}&\texttt{HIP/RF}&{10.73\%$^{\,\,\,}$}&\texttt{RF/GP}&{51.16\%$^{\,\,\,}$}&\texttt{HIP/DT}&{26.55\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/GP}&\cellcolor{red!30}{48.72\%$^\star$}&\texttt{RF/GP}&{21.90\%$^{\,\,\,}$}&\texttt{SVR/GP}&{30.09\%$^{\,\,\,}$}&\texttt{DT/RF}&{15.89\%$^{\,\,\,}$}&\texttt{RF/GP}&{25.96\%$^{\,\,\,}$}\\
\textsc{SQL}&\texttt{DT/RF}&{42.35\%$^{\,\,\,}$}&\texttt{DeP/GP}&{6.70\%$^{\,\,\,}$}&\texttt{DaL/DT}&{12.79\%$^{\,\,\,}$}&\texttt{SVR/GP}&{7.81\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SVR/GP}&{5.05\%$^{\,\,\,}$}&\texttt{GP/RF}&{10.96\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{vp9}&\cellcolor{steel!30}\texttt{RF/RF}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{RF/DT}&{6.54\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{RF/GP}&\cellcolor{red!30}{357.24\%$^\dagger$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{DeP/GP}&{1.43\%$^{\,\,\,}$}&\texttt{SPL/RF}&{39.84\%$^{\,\,\,}$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}\\
\textsc{BDBJ}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{104.79\%$^\star$}&\cellcolor{red!30}\texttt{SPL/GP}&\cellcolor{red!30}{65.51\%$^\star$}&\texttt{RF/DT}&{44.78\%$^{\,\,\,}$}&\texttt{HIP/GP}&{56.98\%$^{\,\,\,}$}&\texttt{SPL/GP}&{36.00\%$^{\,\,\,}$}&\texttt{SVR/GP}&{5.69\%$^{\,\,\,}$}&\texttt{DaL/RF}&{48.51\%$^{\,\,\,}$}&\texttt{SPL/GP}&{35.79\%$^{\,\,\,}$}\\
\textsc{storm}&\cellcolor{red!30}\texttt{GP/RF}&\cellcolor{red!30}{133.46\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/DT}&\cellcolor{red!30}{50.80\%$^\star$}&\texttt{SPL/GP}&{38.13\%$^{\,\,\,}$}&\texttt{SPL/GP}&{49.16\%$^{\,\,\,}$}&\texttt{DeP/GP}&{60.97\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/RF}&\cellcolor{red!30}{349.30\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{91.94\%$^\star$}\\
\textsc{SaC}&\texttt{DeP/RF}&{51.46\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/GP}&\cellcolor{red!30}{81.52\%$^\star$}&\cellcolor{red!30}\texttt{SPL/DT}&\cellcolor{red!30}{109.67\%$^\star$}&\texttt{HIP/GP}&{3.81\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{HIP/GP}&\cellcolor{red!30}{67.30\%$^\star$}&\texttt{SVR/GP}&{10.41\%$^{\,\,\,}$}&\texttt{GP/RF}&{26.48\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DeP/GP}&\cellcolor{red!30}{254.88\%$^\dagger$}\\
\textsc{JavaGC}&\texttt{LR/RF}&{46.78\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{92.69\%$^\star$}&\texttt{RF/DT}&{14.67\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{RF/GP}&\cellcolor{red!30}{530.97\%$^\dagger$}&\cellcolor{red!30}\texttt{LR/GP}&\cellcolor{red!30}{67.99\%$^\star$}&\cellcolor{steel!30}\texttt{GP/GP}&\cellcolor{steel!30}{0.00\%$^{\,\,\,}$}&\texttt{SPL/RF}&{6.10\%$^{\,\,\,}$}&\cellcolor{red!30}\texttt{DaL/GP}&\cellcolor{red!30}{101.74\%$^\star$}\\





\bottomrule
\end{tabular}
\end{adjustbox}

\end{table*}





==> Tables/SMBO.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\caption{SMBO explored in this article}


\begin{adjustbox}{width=\linewidth,center}

\begin{tabular}{llllp{7cm}} 
\toprule
\textbf{SMBO} & \textbf{Feature Selection} & \textbf{Surrogate Model} & \textbf{Acfunc} & \textbf{Acfunc Search Methods} \\ 
\midrule
\texttt{ResTune} & Pre-selection & GP & EI & Numerical optimization \\ 
\rowcolor{steel!10}\texttt{ROBOTune} & Random forest & GP & Hedge & Numerical optimization \\ 
\texttt{Tuneful} & Sensitivity analysis & GP & EI & Numerical optimization \\ 
\rowcolor{steel!10}\texttt{ATConf} & - & GP$_{dropout}$ & LCB & Numerical optimization \\ 
\texttt{OtterTune} & Lasso & GP & LCB & Random sampling and exploration around good configuration \\ 
\rowcolor{steel!10}\texttt{FLASH} & - & DT & Value & All configuration \\ 
\texttt{BOCA} & - & RF & EI & Screened all configuration \\ 
\rowcolor{steel!10}\texttt{SMAC} & - & RF & EI & Random sampling and exploration around good configuration \\ 

\bottomrule

\end{tabular}
\end{adjustbox}
\label{tb:SMBO}
\end{table*}

==> Tables/model_prediction_time.tex <==
\begin{table}[t!]
\centering
\footnotesize
\caption{An instance of one prediction time of surrogate models for system \textsc{SaC}. }
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lllllllllll}
\toprule

& \texttt{SVR}& \texttt{LR}& \texttt{GPR}& \texttt{DT}&\texttt{RF} & \texttt{DECART} & \texttt{SPLConqueror}   & \texttt{DaL} &\texttt{DeepPerf} & \texttt{HINNPerf}\\

\midrule

 Time (ms) & 0.115 & 0.036& 1.636 & 0.035 &3.509   & 0.025 & 0.043   & 0.987 & 0.171  & 1.518  \\

\bottomrule

\end{tabular}
\end{adjustbox}
\label{tb:prediction_time}
\end{table}


==> Tables/models.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\caption{A Summary of Models}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lp{2.3cm}p{2cm}p{4cm}p{4cm}p{2.5cm}l}
\toprule
\textbf{Model} & \textbf{Domain} & \textbf{Applicability} & \textbf{Advantages} & \textbf{Disadvantages}  & \textbf{References/Used by} \\ \midrule
\texttt{SVR} & Machine Learning & General& Addressing high dimensional probelm & High sensitivity to parameter choice and kernel function  & \cite{SVM}/- \\ 
\rowcolor{steel!10}\texttt{LR} & Machine Learning & General& Simple algorithm and fast execution & Only suitable for linear relationships  & \cite{LR}/- \\ 
\texttt{GPR} & Machine Learning & General & Providing uncertainty estimates and high flexibility & Only suitable for low dimension and requiring kernel function selection  & \cite{GPR}/\cite{Ottertune,restune,tuneful,atconf,ROBOTune} \\ 
\rowcolor{steel!10}\texttt{DT} & Machine Learning & General& Handling complex relationships and easy interpretation & Overfitting and instability  & \cite{DT}/\cite{flash} \\ \
\texttt{RF} & Machine Learning & General& Managing complex relationships, high accuracy and stability & Complexity and interpretability challenges  & \cite{RF}/\cite{BOCA,SMAC} \\ 
\rowcolor{steel!10}\texttt{DECART} & Machine Learning & General& Handling non-linear and complex relationships & Overfitting  & \cite{DECART}/- \\ 
\texttt{SPLConqueror} & Machine Learning & Configurable systems& Efficiently handling complex relationships & Computational cost is relatively high  & \cite{SPL}/- \\ 
\rowcolor{steel!10}\texttt{DaL} & Machine/Deep Learning & Configurable systems& Efficiently addressing feature sparsity & High data requirements and black-box nature  & \cite{DaL}/- \\ 
\texttt{DeepPerf} & Deep Learning & Configurable systems& High accuracy for binary and/or numeric configurations & High data requirements and black-box nature  & \cite{DeepPerf}/- \\ 
\rowcolor{steel!10}\texttt{HINNPerf} & Deep Learning & Configurable systems& High accuracy through hierarchical modeling & High data requirements and black-box nature  & \cite{HINNPerf}/- \\ \bottomrule
% \texttt{Perf-AL} & Deep Learning & High accuracy with minimal training samples & High data requirements and black-box nature & Highly Configurable Systems & \cite{PerfAL}/- \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:models}
\end{table*}


==> abstract.tex <==
\begin{abstract}
 Configuring hyperparameters is an important part of using various software systems. Among them, automated hyperparameter tuning aims to automate this process using search algorithms which mainly includes sequential model-based optimization (SMBO) and model-free optimization (MFO). In the former, the choice of the surrogate model has a huge impact on the optimization process and performance. In the latter, using a model to substitute the real space which we call it batch model-based optimization (BMBO) also greatly affects the process and outcomes. Having known the key position of the model, to investigate the model's influence, although there are different optimizer using alternative models, they are just specific combinations. We still know little about effect of the model accuracy to the optimization efficiency and performance. 
 
 To fill this gap, this paper empirically analyzes and compares the results of eight SMBO and eight MFO of ten types of models under 24 different systems, with a total of 3,840 cases. Our key findings reveals that: (1) SMBO with surrogate model selected outperforms MFO bench and BMBO lose in performance but almost tie with MFO bench in efficiency; (2) The majority (over 81\%) of the widely used SMBO with systems can make progress by changing the model; (3) The positive correlation of model accuracy with optimization results in BMBO is significant, while the positive correlation in SMBO is weak and there are even numerous bad effect of high model accuracy. Alongside our findings, we also provide some practical suggestion and guidance which includes how to choose the model and how to improve performance and efficiency compared with the original model.

\end{abstract}

==> main-old.tex <==
% %%
% %% This is file `sample-acmsmall.tex',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% samples.dtx  (with options: `acmsmall')
% %% 
% %% IMPORTANT NOTICE:
% %% 
% %% For the copyright see the source file.
% %% 
% %% Any modified versions of this file must be renamed
% %% with new filenames distinct from sample-acmsmall.tex.
% %% 
% %% For distribution of the original source see the terms
% %% for copying and modification in the file samples.dtx.
% %% 
% %% This generated file may be distributed as long as the
% %% original source files, as listed above, are part of the
% %% same distribution. (The sources need not necessarily be
% %% in the same archive or directory.)
% %%
% %% Commands for TeXCount
% %TC:macro \cite [option:text,text]
% %TC:macro \citep [option:text,text]
% %TC:macro \citet [option:text,text]
% %TC:envir table 0 1
% %TC:envir table* 0 1
% %TC:envir tabular [ignore] word
% %TC:envir displaymath 0 word
% %TC:envir math 0 word
% %TC:envir comment 0 0
% %%
% %%
% %% The first command in your LaTeX source must be the \documentclass command.
% \documentclass[acmsmall]{acmart}
% %% NOTE that a single column version is required for 
% %% submission and peer review. This can be done by changing
% %% the \doucmentclass[...]{acmart} in this template to 
% %% \documentclass[manuscript,screen]{acmart}
% %% 
% %% To ensure 100% compatibility, please check the white list of
% %% approved LaTeX packages to be used with the Master Article Template at
% %% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
% %% before creating your document. The white list page provides 
% %% information on how to submit additional LaTeX packages for 
% %% review and adoption.
% %% Fonts used in the template cannot be substituted; margin 
% %% adjustments are not allowed.
% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2018}
% \acmYear{2018}
% \acmDOI{XXXXXXX.XXXXXXX}


% %%
% %% These commands are for a JOURNAL article.
% \acmJournal{JACM}
% \acmVolume{37}
% \acmNumber{4}
% \acmArticle{111}
% \acmMonth{8}
% % \usepackage{subcaption}
% \usepackage{pgf-pie}
% \usepackage{xcolor} 
% \usepackage{subfig}
% \usepackage{pgfplots}
% \usepackage{pgfplotstable}
% \usepackage{adjustbox}
% \usepackage{booktabs}
% \usepackage{csquotes}
% \usepackage{geometry}
% \usepackage{multirow}
% \usepackage[figuresright]{rotating}
% \usepackage{tcolorbox}
% \usepackage{colortbl}
% \usepackage{xcolor}
% \DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}


% \definecolor{steel}{rgb}{0, 0.2, 0.9} 

% \newtcolorbox{quotebox}{colback=black!10,boxrule=0.4pt,colframe=black,fonttitle=\bfseries,top=2pt,bottom=2pt}

% \input{tablefigures}
% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% For managing citations, it is recommended to use bibliography
% %% files in BibTeX format.
% %%
% %% You can then either use BibTeX with the ACM-Reference-Format style,
% %% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
% %% support for advanced citation of software artefact from the
% %% biblatex-software package, also separately available on CTAN.
% %%
% %% Look at the sample-*-biblatex.tex files for templates showcasing
% %% the biblatex styles.
% %%

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}

% %%
% %% end of the preamble, start of the body of the document source.
% \begin{document}

% %%
% %% The "title" command has an optional parameter,
% %% allowing the author to define a "short title" to be used in page headers.
% %\title{Is Model Accuracy Useful? An Empirical Study on Models for Knob Tuning}
% \title{Accuracy can Lie: On the Impact of Surrogate Model in Configuration Tuning}

% %%
% %% The "author" command and its associated commands are used to define
% %% the authors and their affiliations.
% %% Of note is the shared affiliation of the first two authors, and the
% %% "authornote" and "authornotemark" commands
% %% used to denote shared contribution to the research.
% \author{Pengzhou Chen}
% % \authornote{Both authors contributed equally to this research.}
% \email{trovato@corporation.com}
% % \orcid{1234-5678-9012}
% \author{Tao Chen}
% \authornotemark[1]
% \email{webmaster@marysville-ohio.com}
% \affiliation{%
%   \institution{University of Electronic Science and Technology of China}
%   % \streetaddress{P.O. Box 1212}
%   \city{Chengdu shi}
%   \state{Sichuan sheng}
%   \country{China}
%   % \postcode{43017-6221}
% }

% \author{Jingzhi Gong}
% \affiliation{%
%   \institution{Loughborough University}
%   % \streetaddress{streetaddress}
%   \city{Loughborough}
%   \country{UK}}
% \email{j.gong@lboro.ac.uk}

% %%
% %% By default, the full list of authors will be used in the page
% %% headers. Often, this list is too long, and will overlap
% %% other information printed in the page headers. This command allows
% %% the author to define a more concise list
% %% of authors' names for this purpose.
% \renewcommand{\shortauthors}{Trovato and Tobin, et al.}

% %%
% %% The abstract is a short summary of the work to be presented in the
% %% article.
% \input{abstract}

% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%        <concept_id>10011007.10011074.10011784</concept_id>
%        <concept_desc>Software and its engineering~Search-based software engineering</concept_desc>
%        <concept_significance>500</concept_significance>
%        </concept>

%    <concept>
%        <concept_id>10011007.10011074.10011099.10011693</concept_id>
%        <concept_desc>Software and its engineering~Empirical software validation</concept_desc>
%        <concept_significance>300</concept_significance>
%        </concept>
       
%           <concept>
%        <concept_id>10011007.10010940.10011003.10011002</concept_id>
%        <concept_desc>Software and its engineering~Software performance</concept_desc>
%        <concept_significance>300</concept_significance>
%        </concept>
%  </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Software and its engineering~Search-based software engineering}
% \ccsdesc[300]{Software and its engineering~Empirical software validation}
% \ccsdesc[300]{Software and its engineering~Software performance}
% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% \keywords{Search-based software engineering, software configuration tuning, sequential model-based optimization, configurable systems, heuristic methods.}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

% %%
% %% This command processes the author and affsiliation and title
% %% information and builds the first part of the formatted document.
% \maketitle



% \input{introduction}

% \input{background}

% \input{methodology}

% \input{results}

% \input{Lessons Gained}

% \input{threats to validity}

% \input{related}

% \input{conclusion}


% % \section{CCS Concepts and User-Defined Keywords}

% % Two elements of the ``acmart'' document class provide powerful
% % taxonomic tools for you to help readers find your work in an online
% % search.

% % The ACM Computing Classification System ---
% % \url{https://www.acm.org/publications/class-2012} --- is a set of
% % classifiers and concepts that describe the computing
% % discipline. Authors can select entries from this classification
% % system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
% % commands to be included in the \LaTeX\ source.

% % User-defined keywords are a comma-separated list of words and phrases
% % of the authors' choosing, providing a more flexible way of describing
% % the research being presented.

% % CCS concepts and user-defined keywords are required for for all
% % articles over two pages in length, and are optional for one- and
% % two-page articles (or abstracts).





% % \section{Acknowledgments}

% % Identification of funding sources and other support, and thanks to
% % individuals and groups that assisted in the research and the
% % preparation of the work should be included in an acknowledgment
% % section, which is placed just before the reference section in your
% % document.

% % This section has a special environment:
% % \begin{verbatim}
% %   \begin{acks}
% %   ...
% %   \end{acks}
% % \end{verbatim}
% % so that the information contained therein can be more easily collected
% % during the article metadata extraction phase, and to ensure
% % consistency in the spelling of the section heading.

% % Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

% % \section{Appendices}

% % If your work needs an appendix, add it before the
% % ``\verb|\end{document}|'' command at the conclusion of your source
% % document.

% % Start the appendix with the ``\verb|appendix|'' command:
% % \begin{verbatim}
% %   \appendix
% % \end{verbatim}
% % and note that in the appendix, sections are lettered, not
% % numbered. This document has two appendices, demonstrating the section
% % and subsection identification method.

% % \section{Multi-language papers}

% % Papers may be written in languages other than English or include
% % titles, subtitles, keywords and abstracts in different languages (as a
% % rule, a paper in a language other than English should include an
% % English title and an English abstract).  Use \verb|language=...| for
% % every language used in the paper.  The last language indicated is the
% % main language of the paper.  For example, a French paper with
% % additional titles and abstracts in English and German may start with
% % the following command
% % \begin{verbatim}
% % \documentclass[sigconf, language=english, language=german,
% %                language=french]{acmart}
% % \end{verbatim}

% % The title, subtitle, keywords and abstract will be typeset in the main
% % language of the paper.  The commands \verb|\translatedXXX|, \verb|XXX|
% % begin title, subtitle and keywords, can be used to set these elements
% % in the other languages.  The environment \verb|translatedabstract| is
% % used to set the translation of the abstract.  These commands and
% % environment have a mandatory first argument: the language of the
% % second argument.  See \verb|sample-sigconf-i13n.tex| file for examples
% % of their usage.

% % \section{SIGCHI Extended Abstracts}

% % The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
% % not in Word) produces a landscape-orientation formatted article, with
% % a wide left margin. Three environments are available for use with the
% % ``\verb|sigchi-a|'' template style, and produce formatted output in
% % the margin:
% % \begin{itemize}
% % \item {\verb|sidebar|}:  Place formatted text in the margin.
% % \item {\verb|marginfigure|}: Place a figure in the margin.
% % \item {\verb|margintable|}: Place a table in the margin.
% % \end{itemize}

% %%
% %% The acknowledgments section is defined using the "acks" environment
% %% (and NOT an unnumbered section). This ensures the proper
% %% identification of the section in the article metadata, and the
% %% consistent spelling of the heading.
% % \begin{acks}
% % To Robert, for the bagels and explaining CMYK and color spaces.
% % \end{acks}

% %%
% %% The next two lines define the bibliography style to be used, and
% %% the bibliography file.
% \bibliographystyle{ACM-Reference-Format}
% \bibliography{reference}

% %%
% %% If your work has an appendix, this is the place to put it.
% % \appendix

% % \section{Research Methods}

% % \subsection{Part One}

% % Lorem ipsum dolor sit amet, consectetur adipiscing elit. Morbi
% % malesuada, quam in pulvinar varius, metus nunc fermentum urna, id
% % sollicitudin purus odio sit amet enim. Aliquam ullamcorper eu ipsum
% % vel mollis. Curabitur quis dictum nisl. Phasellus vel semper risus, et
% % lacinia dolor. Integer ultricies commodo sem nec semper.

% % \subsection{Part Two}

% % Etiam commodo feugiat nisl pulvinar pellentesque. Etiam auctor sodales
% % ligula, non varius nibh pulvinar semper. Suspendisse nec lectus non
% % ipsum convallis congue hendrerit vitae sapien. Donec at laoreet
% % eros. Vivamus non purus placerat, scelerisque diam eu, cursus
% % ante. Etiam aliquam tortor auctor efficitur mattis.

% % \section{Online Resources}

% % Nam id fermentum dui. Suspendisse sagittis tortor a nulla mollis, in
% % pulvinar ex pretium. Sed interdum orci quis metus euismod, et sagittis
% % enim maximus. Vestibulum gravida massa ut felis suscipit
% % congue. Quisque mattis elit a risus ultrices commodo venenatis eget
% % dui. Etiam sagittis eleifend elementum.

% % Nam interdum magna at lectus dignissim, ac dignissim lorem
% % rhoncus. Maecenas eu arcu ac neque placerat aliquam. Nunc pulvinar
% % massa et mattis lacinia.

% \end{document}
% \endinput
% %%
% %% End of file `sample-acmsmall.tex

==> methodology-old.tex <==
\section{Research Methodology}
\label{sec:methodology}

We now delineate the methodology of our empirical study.



\subsection{System and Data}
In this empirical study, to enhance the generality of the results, we chose the systems that has been widely used in multiple different domains and with varying data volumes. Table~\ref{tb:dataset} presents key data for each system, including budget, space size, domain, and the number of parameters. Additionally, the dataset encompasses various systems and software, such as database systems, data compression software, web application servers, and machine learning hyperparameter optimization.




For the subsequent research, we divided the data into two categories: large datasets and small datasets. The classification criterion was based on the size of the data search space[]. When the number of configurations in the search space exceeded $1\times10^6$, we refer to it as a large system. Otherwise, it is categorized as a small system.


\subsection{Architecture of the experiments}
\subsubsection{Trade off between Exploitation and Exploration}\label{sec:3.2.1}


Trading off between exploitation and exploration is typically achieved through the use of acquisition functions, which is a crucial component of SMBO. Common acquisition functions include:
\begin{itemize}

\item \textbf{Probability of Improvement (PI)} calculates the probability of improving the current best solution by sampling a new point \cite{PI}.
\item \textbf{Expected Improvement (EI)} is based on the current model's predicted values and prediction uncertainty, estimating the expected improvement over the current best value \cite{EI}.
\item \textbf{Upper Confidence Bound (UCB)} is based on the current model's predicted values and prediction uncertainty, selecting the upper confidence bound as the acquisition criterion \cite{UCB}.
\end{itemize}

In each iteration of SMBO, the goal is to select the real best configuration to be trained in the model. The acquisition function evaluates the rewards of selected candidates in each iteration, and the best candidate is chosen based on this evaluation. The performance of the selected candidate is then measured in the real system, and the configuration is added to the training set to guide the search for the overall best configuration.

The acquisition function faces a trade-off between exploitation and exploration. Exploitation focuses on the depth of sampling, ensuring that the model predicts candidate values more accurately. To achieve deep exploration, the model must be able to predict candidate values, a requirement that the models we use can meet. Exploration, on the other hand, emphasizes the breadth of sampling, trying to explore as many unknown areas as possible. To achieve exploration, the model needs to provide a measure of uncertainty at candidates.

\texttt{GP} and \texttt{RF} are models that have been successfully used in the past, among which \texttt{GP} directly models the mean and variance, allowing itself to output the variance at candidate points as a measure of uncertainty. \texttt{RF} employs bagging on the data, building multiple \texttt{DT} models across various subsets, using the variance of multiple predictions of \texttt{DT} as the measure of uncertainty.

Inspired by the approach of \texttt{RF}, we adopt a similar method to handle models that cannot directly output uncertainty. Firstly, we perform bagging on the training set to generate multiple subsets and then use these subsets to train multiple sub-models. Finally, we use the variance of predictions from the sub-models as the measure of uncertainty, with the output of the model trained on the whole data as the final prediction value. This approach ensures both prediction stability and provides a measure of uncertainty of each model.

\subsubsection{Hyperparameters: Initial Size, Tuning Budget, and Training Budget}

After selecting various algorithms, from their original papers and open-source code, we discovere that different algorithms employed distinct initial sizes (MFO did not have an initial size) and tuning budgets to address various systems to be optimized. Initial size and tuning budget are among the most critical parameters to select within SMBO and training budget is significant in MFO. To determine these parameters, we adopt the following methods.
\begin{itemize}
 

\item\textbf{{Initial Size}}
is the number of configurations selected initially for model training. A larger initial size means that more configurations are selected initially, allowing for a more precise initialization of the model and, consequently, being more favorable for finding new configurations. However, an increased initial size also comes with higher costs and when the budget is fixed, increasing initial size potentially lead to decreased chances of finding better performance.

In SMBO, authors of the SMBO papers chose various initial sizes, including 1 (\texttt{ATConf}), 2 (\texttt{BOCA}), 5 (\texttt{OtterTune}), 10 (\texttt{ResTune}), and 20 (\texttt{FLASH}, \texttt{ROBOTune}). We opt for an initial size of 20 for the following reasons: initial sizes of 1, 2, and 5 were excluded from our selection due to the dataset being too small for training, which rendered additional models, such as \texttt{DaL}. Therefore, only the initial sizes of 10 and 20 are considered. Then we select the initial size of 20 due to its greater usage frequency.

\item\textbf{{Tuning Budget}}
represents the allocation for finding the optimal performance of a given system, which means that we can measure different configurations for that number of times. A larger budget implies more measurements and the ability to explore a broader range of configurations, which increases the opportunity to find better performance. However, determining the budget is not straightforward, as our empirical study included different systems, optimizers and models, each of which had unforeseeable effects on the required training convergence.

To address this issue, we adopt an adaptive and dynamic approach to determine the budget. To ensure fairness, all algorithms for the same system needed to employ the same budget. The method was inspired by the idea that different algorithms, regardless of their type, would find their best performance after a certain budget, after which there would be no improvement for a long time. The actual budget is the number of different configurations measured. To facilitate comparison, a suitable budget should be chosen to ensure that all algorithms have reached a convergence state.

Therefore, we conducted Pre-experiments in which we set a lives limit of one hundred iterations. If an algorithm failed to find better performance after one hundred iterations, it was considered converged. Subsequently, we measured the budgets for all algorithms and select the maximum value of the budget among all the algorithms for specific system. This approach ensure that all algorithms have reached the convergence state and that the algorithms do not conduct excessive useless searches. The selection of the budget was performed across five random seeds to improve the generality of the results.

\item\textbf{{Training Budget}}
is an essential hyperparameter in BMBO because we need to fit the pre-trained model into these algorithms. To determine this size, we refer to the approach taken by \cite{siegmund2015performance}. The sampling method focuse on distinguishing binary options and numerical options and employ different sampling methods tailored to their characteristics, subsequently combining them to obtain comprehensive configuration sampling. 

We classified the knobs into binary and non-binary categories and applied option\_wise sampling or pair\_wise sampling and Plackett Burman design sampling or random design methods for each knob category. Simultaneously, we employed Plackett Burman design sampling with two sets of parameters, resulting in six sample sizes finally. Among these sizes, we choose the largest sample size to ensure that the model received adequate training, facilitating the exploration of accuracy differences between different models and contributing to the exploration of final performance differences.


\end{itemize}



\subsubsection{Workflow}
With the knowledge provided above, we now introduce the entire experimental process. 
% Figure [] reveals the workflow of our experiment. 
The implementation of the experiment can be summarized in the following steps:

\textbf{1) Pre-experiments}
\begin{itemize}
   \item[a.] Since the size and feature of the system vary, the required tuning budget to achieve stability differs. Therefore, the experiment starts with a pre-experiment to determine the unique budget needed for each different system within SMBO and MFO.
   \item[b.] Similarly, due to the varying space sizes for each system, we need to compute different budgets to pre-trained models, which will later be integrated into BMBO.
\end{itemize}

\textbf{2) Formal Experiments}
\begin{itemize}
   \item[a.] For eight SMBO, we replace their models by integrating the ten different models mentioned in section~\ref{sec:models} into these optimization frameworks. We use the initial size and tuning budget determined during the discussions and pre-experiment phase. Note that we employ the same tuning budget for the same system in all optimization frameworks and we make no changes to the other parts of the framework to ensure that the results are not influenced by other factors.
  \item[b.] For nine BMBO, we substitute their models by incorporating all ten different pre-trained models into these optimization frameworks. Then, we use the tuning budget obtained and the model that has been trained during the pre-experiment stage to conduct BMBO.
   \item[c.] For nine MFO, there is no need to use models and we conduct MFO in two tuning budget. One of them is the tuning budget for comparison with SMBO, and the other is the training budget of pre-trained model for comparison with BMBO, which ensures the consistency of exploring real space.

\end{itemize}





\subsection{Metrics and Statistical Validation}
This part presents the metrics and statistical validation used later to measure and validate our results. 
\subsubsection{Metrics}

This study is to investigate the impact of model accuracy. To achieve this, we need to utilize several metrics for evaluating and quantifying the accuracy. The primary function of the model is to predict candidates and select configurations with relatively better performance using an acquisition function. Hence, we need to focus on both the actual accuracy and the relative ranking accuracy of the models ,so we choose metrics for accuracy measurement from two distinct  perspectives.\

\textbf{1) Mean Absolute Percentage Error ($MAPE$)} 


 $MAPE$ is a percentage error metric that calculates the percentage of absolute errors relative to the actual values. By normalizing the relative magnitude of errors, it facilitates the comparison of performance across various problem domains, independent of the system range. $MAPE$ is calculated as:

\begin{equation}
MAPE = \frac{1}{n} \sum_{i=1}^{n} \left|\frac{y_i - \hat{y}_i}{y_i}\right| \cdot 100\% 
\label{eq:MAPE}
\end{equation}
where $n$ is the number of samples and $y_i$ corresponds to the true target value of the $i$-th sample. $\hat{y}_i$ represents the predicted value of the $i$-th sample. The formula quantifies the average percentage error between the predicted values and the actual values, providing a standardized measure of error relative to the actual data and it is particularly useful for comparing model performance across different systems.

\textbf{2) Mean Rank Difference ($\mu RD$)} 

$\mu RD$ is used to calculate the number of pairs in the test data where the performance model ranks them incorrectly and measures the average rank difference. This metric focuses on the accuracy of the ranking of predictions. For the sake of standardizing units, we have additionally divided the efficiency by the sample size to eliminate the influence of sample size on the results \cite{flash}. The calculation of µRD is as equation~(\ref{eq:MURD}) :

\begin{equation}
\mu RD = \frac{1}{n^2} \sum_{i=1}^{n} (rank(y_i) - rank(\hat{y}_i))
\label{eq:MURD}
\end{equation}
in which $n$ signifies the number of samples, $y_i$ corresponds to the true target value of the $i$-th sample and $\hat{y}_i$ stands for the predicted value for the $i$-th sample. The choice of $n$ being a square is to eliminate the influence of data volume, maintaining comparability across different systems.


\textbf{3) Efficiency}


In optimization, We also need to consider the efficiency of the progressively predicted models. According to \cite{chen2021multi}, we can use $r$ to measure the efficiency of the models and the calculation of $r$ is as follows:
\begin{equation}
r = \frac{m}{b} \cdot 100\%
\label{eq:r}
\end{equation}
whereby $m$ represents the smallest budget consumed by methods to achieve the same or better target performance objective and $b$ is the smallest number of measurements that the worst optimizer consumes to achieve its best result. The choice of target performance is a critical parameter that influences the results, and we determine the target performance by self-adaption.


\textbf{4) Improvement}

To assess the disparity between the proposed method and the baseline, the metric Impr. is defined as:

\begin{equation}
    Impr. = \frac{X-X_{\text {baseline }}}{X_{\text {baseline }}} \cdot 100 \%
\label{eq:Impr.}
\end{equation}
whereby X can be performance or efficiency of different SMBO or BMBO which implies the difference from the baseline.



\subsubsection{Statistical Validation}\label{sec:3.3.2}

We primarily utilize three tests, details are as follows.

\textbf{1) Mann-Whitney U-Test}

In order to assess whether there is a significant difference between two sets of sample values, we use Mann-Whitney U-Test for comparing the medians of two sets.
\begin{enumerate}
\item Initially, combine two sets of data and rank the data based on their magnitudes.
\item Compare whether there is a significant difference in the medians of the two groups by calculating the sum of ranks. 
\end{enumerate}

% We use a 95\% confidence level as the confidence interval for significant differences.

\textbf{2) Spearman's Rank Correlation Test}

Spearman's Rank Correlation Test is a non-parametric statistical test used to assess the monotonic relationship between two variables. We need to explore the monotonic relationship between two variables, and performing the test can be broadly outlined in the following steps:
\begin{enumerate}
  \item Rank the observed values: sort the observed values for each variable and convert them into ranks.
  \item Calculate rank differences: for each pair of paired ranks, calculate their differences.
  \item Utilize the calculated rank differences to compute the Spearman's rank correlation coefficient.
  \item Hypothesis testing: Use the calculated Spearman's rank correlation coefficient for hypothesis testing to determine whether the observed correlation is significant. 
\end{enumerate}

The Spearman's rank correlation coefficient ranges from -1 to 1. A positive value indicates a monotonically increasing relationship, while a negative value indicates a monotonically decreasing relationship. A value of 0 signifies the absence of a monotonic relationship. The significance level, also referred to as the p-value, is utilized to assess whether the observed correlation is the result of random chance or a meaningful pattern.

\textbf{3) Scott-Knott Effect Size Difference (ESD) Test}

The Scott-Knott ESD test represents a method for comparing means, employing hierarchical clustering to partition sets of means into statistically distinct groups that exhibit highly significant differences. We do Scott-Knott ESD test as follows:

\begin{enumerate}
  \item Groups are sorted based on the mean effect, and the sum of squares between groups is calculated to identify a partition that maximizes treatment means between groups.
  \item The magnitude of the difference is then analyzed for each pair of treatment means across the two groups. If a non-negligible difference is observed in any pair of treatment means between two groups, they are separated into two distinct groups. Conversely, if the differences are negligible across all pairs, the groups are merged into a single cohesive group.
 
\end{enumerate}

For instance, considering the sorting of groups A, B, C and D, the final arrangement may be delineated as follows: first group (A, D), second group (B), and third group (C).

==> novelty_statement.tex <==
% \documentclass[a4paper,11pt]{article}

% \usepackage{csquotes}
% %\usepackage{longtable}
% %\signature{Dr.~Denis Demidov}
% %\address{
% %Joint Supercomputer Center \\
% %Russian Academy of Sciences \\
% %Lobachevsky st. 2/31\\
% %420111 Kazan, Russia \\
% %email: ddemidov@ksu.ru
% %}
% \begin{document}

% %\begin{letter}{
% %    Hans Petter Langtangen\\
% %    Editor-in-Chief\\
% %    SIAM Journal of Scientific Computing
% %    }
% %\opening{Dear Dr.~Langtangen,}

% \begin{flushleft} 
% Dear Editor-in-Chief, Associate Editor and Reviewers,
% \end{flushleft} 


% We hereby declare that the submitted manuscript satisfy the following criteria for Journal-First submission:

% \begin{itemize}

% \item It reports completely new research results or else it presents novel contributions that significantly extend and were not previously reported in prior work.

% \item It does not extend prior work solely with additional proofs or algorithms or other such details presented for completeness, or additional empirical results, or minor enhancements or variants of the results presented in the prior work.

% \end{itemize}

% %\closing{Sincerely,}

% \vspace{-1cm}
% \begin{flushleft} 
% \vspace{1cm}
% Sincerely yours, \\
% \vspace{1cm}
% Pengzhou Chen, Jingzhi Gong and Tao Chen

% \end{flushleft} 

% %\end{letter}

% %\bibliographystyle{abbrv}
%  %argument is your BibTeX string definitions and bibliography database(s)
% %\bibliography{references}

% % \\ \hline
% %
% % \hline \hline
% %
% %\end{longtable}

% \end{document}

==> results-RQ1-3.tex <==
\section{Results and Analysis}
\label{sec:results}

In this section, we summarize and discuss the results obtained.
%with RQ1, we need to say how difficult is it to directly compare sequential and batch, and say they can be compared via model free indrectly

\subsection{RQ1: How Useful is the Model for Tuning Quality?}
\label{sec:rq1}

%for RQ1.1, talk about not really the best is the original model

%for RQ1.2, there should not be equal the the original, but the difference between the original and the best, so we compare original with the best except the original

% need to highlight the best per system, e.g., use underline

\subsubsection{Method}

To answer \textbf{RQ1}, we respectively compare the sequential and batch model-based tuners, paired with all possible models, against their model-free counterparts. Since there are many tuner-model pairs and model-free tuners to compare, for each system, we select the best representative from each tuner type. To that end, we run Scott-Knott ESD test on each tuning quality metric, and use the one that is ranked the first as the representative; if there is more than one pair/tuner in the best rank, we choose the one with the best average quality. It is worth noting that, when comparing model-free tuners with sequential model-based tuners, they are set with the budget identified in Section~\ref{sec:size}. In contrast, when comparing them with batch model-based tuners, their budget is set as the same as the training sample size used by the batch model-based ones, which is already a large figure compared with existing work. This is because only the measurement of systems is expensive in configuration tuning while the other factors are relatively marginal, hence matching them in that aspect ensures a fairer comparison. Since there are 29 systems, we have 29 cases under each metric.



The pairwise comparisons are verified by the Mann-Whitney U-test. All other settings are the same as discussed in Section~\ref{sec:methodology}. Any statistically insignificant comparisons are regarded as ties.

\begin{figure}[t!]
\centering
%\includegraphics[width=0.3\columnwidth]{Figures/rq1.1-summary-legend.pdf}
\subfloat[sequential vs. model-free]{\includestandalone[width=0.49\columnwidth]{Figures/rq1.1-summary-1}}
~\hfill
\subfloat[batch vs. model-free]{\includestandalone[width=0.49\columnwidth]{Figures/rq1.1-summary-2}}

\caption{Comparing the best tuner-model pair against the best model-free tuner under each system for all 29 cases (30 runs). We count how many cases the best tuner-model pair wins, loses, or ties.}
\label{fig:rq1.1-sum}
\end{figure}
 

\subsubsection{Results}

From Figure~\ref{fig:rq1.1-sum}, for sequential model-based tuner, it is clear that the models are overwhelmingly helpful against the counterpart when the model is absent. Even with the statistical test, out of the 29 cases, the sequential model-based tuner still wins over the model-free counterpart on 16 cases; draws on 10, and loses only on 3 in terms of performance. For efficiency, the best model-tuner pair has a remarkable win on 21 cases with 6 and 2 cases of tie and loss, respectively. Looking at the detailed results in Table~\ref{tb:rq1.1}, the model can help the sequential model-based tuner to achieve a maximum of 160\% performance improvement and up to $50\times$ better for efficiency. 

\input{Tables/RQ4/SMBO}
\input{Tables/RQ4/MFO}

We also found that the best tuner-model pair for the sequential model-based tuners is system-dependent for both performance and efficiency; the same applies to the model-free tuners. However, \texttt{Flash} and \texttt{SMAC}/\texttt{ROBOTune} appear to be often part of the best tuner-model pair for performance and efficiency, respectively. For the model-free counterparts, both the \texttt{BestConfig} and \texttt{ParamILS} tend to be more competitive than the others.

The divergence of tuning quality between the two types of tuner appears to be larger on small systems (e.g., \textsc{Brotli}) than the others. This is possible since being small in terms of the search space does not necessarily mean that they are simple, because the landscape can still be radically complex to be modeled and contain many local optima traps.

\begin{tcbitemize}[%
    raster columns=1, 
    raster rows=1
    ]
  \tcbitem[myhbox={}{Finding \thefindingcount}]   \textit{Models can considerably improve the sequential model-based tuner over its model-free counterpart in 16 (up to 160\% improvement) and 21 (up to $5\times$ better) out of 29 cases for performance and efficiency, respectively, demonstrating its usefulness in guiding the tuning when they can be continuously updated.}
\end{tcbitemize}
\addtocounter{findingcount}{1}

In contrast, we observe rather different results when comparing batch model-based tuners with the model-free ones. From Figure~\ref{fig:rq1.1-sum}, we see that the best tuner-model pair from the batch type is commonly worse than the best model-free counterpart for performance. While it appears to be better than model-free tuner in efficiency, the improvements are often not statistically significant. In particular, the batch model-based tuner loses 28 cases with 1 tie for performance; it wins 6 cases and loses 1 case, together with 22 ties, for efficiency. The detailed results in Table~\ref{tb:rq1.2} show that the degradation of batch model-based tuner over the model-free one can be up to 200\%. Such a discrepancy, compared with the results of sequential model-based tuners, is due to the fact that the models are not updated progressively during tuning when used for batch model-based tuners.





As for the generally best tuner-model pair under batch model-based tuners, again, we found no generally best one across the systems. For both types of tuners, the \texttt{BestConfig} and \texttt{ParamILS} remain robust on both tuning quality metrics. Again, the quality divergence tends to be larger on the small systems compared with the others due to the same reason mentioned before.


\begin{tcbitemize}[%
    raster columns=1, 
    raster rows=1
    ]
  \tcbitem[myhbox={}{Finding \thefindingcount}]  \textit{Conversely, models generally have marginal or even harmful impact on the tuning quality of batch model-based tuner, as out of the 29 cases, they lose on 28 cases on performance while drawing or losing on 24 cases for efficiency against the model-free one.}
\end{tcbitemize}
\addtocounter{findingcount}{1}



% comparing sequential and batch?








%\subsection{RQ2: To What Extent Does the Best/Worst Model Accuracy Match with the Expected Tuning Quality?}


\subsection{RQ2: DO the Chosen Models Work the Best on Tuning Quality?}

\subsubsection{Method}


Another interesting investigation related to the model usefulness is to explore whether the fixed model, originally chosen for sequential model-based tuners (so-called origin), is indeed the optimal setting in terms of tuning quality, e.g., whether the \textsc{CART} used in \textsc{FLASH} is the best option. To that end, under each combination of system and tuner, we compare the best representative from all tuner-model pairs (selected in the same way as \textbf{RQ1} according to a quality metric) against the original tuner-model pair. In total, we have 29 systems $\times$ 8 sequential model-based tuners $=232$ cases to discuss for each metric. Other settings are the same as \textbf{RQ1}.




\subsubsection{Results}

Surprisingly, from Figure~\ref{fig:rq1.2-sum}, we see that the origins in sequential model-based tuners are often not as effective as we expected, as compared with some arbitrarily new tuner-model pairs, they lose on 46\% of the cases (106/232) with 50\% tie (116/232) on performance. Similar results can also be observed for efficiency: the origin has 32\% (74/232 cases) loss and 66\% (153/232 cases) tie.

Specifically, Tables~\ref{tb:rq2.1} and~\ref{tb:rq2.2} show the detailed results on different systems. Clearly, the performance can be improved by up to 286.62\% when we simply replace \texttt{OtterTune}'s \texttt{GP} with \texttt{DECART} under \textsc{kanzi}. Likewise, the efficiency improvement can reach up to 699.63\% by modifying \texttt{OtterTune}'s \texttt{GP} to \texttt{DaL} under \textsc{ExaStencils}. All of the above suggests that the originally chosen tuner-model pairs for sequential model-based tuners are far away from being optimal on any single metric of the tuning quality.

We also see that, relatively, the tuning quality of certain tuners can be more significantly improved by replacing the original model. This means that the impact of model replacement depends on the tuner's nature, e.g., \texttt{OtterTune} relies on gradient descent that works on the landscape predicted by the model to explore the configuration space, thereby any subtle change of the landscape caused by the model replacement can be much more influential to its behaviors. We also observe that there has been no consistent pattern regarding the systems, as the models can be sensitive to the characteristics of configuration data, e.g., sparsity.



\begin{figure}[t!]
\centering
\subfloat[performance]{\includestandalone[width=0.49\columnwidth]{Figures/rq1.2-summary-1}}
~\hfill
\subfloat[efficiency]{\includestandalone[width=0.48\columnwidth]{Figures/rq1.2-summary-2}}

\caption{Comparing the original model in the sequential model-based tuner against the best alternative model when tuning under each combination of system and tuner for all 232 cases (30 runs). We count how many cases the origin wins, loses, or ties.}
\label{fig:rq1.2-sum}
\end{figure}
% talk about system/tuner specifics?

\begin{tcbitemize}[%
    raster columns=1, 
    raster rows=1
    ]
  \tcbitem[myhbox={}{Finding \thefindingcount}]  \textit{The original model used in sequential model-based tuners has marginal difference or can be significantly improved (for over 95\% of the cases) compared with some other, ``newly created'' tuner-model pairs.}
\end{tcbitemize}
\addtocounter{findingcount}{1}



\input{Tables/RQ5/SMBO1}
\input{Tables/RQ5/SMBO2}


\begin{figure}[t!]
\centering
\subfloat[sequential model-based tuners]{\includestandalone[width=0.49\columnwidth]{Figures/rq3-summary-smbt}}
~\hfill
\subfloat[batch model-based tuners]{\includestandalone[width=0.49\columnwidth]{Figures/rq3-summary-bmbt}}

\caption{Counting the number of cases where the best (worst) model chosen based on accuracy matches with the model that leads to the best (worst) tuning quality with 30 repeats. $\mathcal{B}$ and $\mathcal{W}$ refer to the scenario of best and worst representative, respectively. M\&P, R\&P, M\&E, and R\&E respectively denote the combined metric set of MAPE-performance, $\mu$RD-performance, MAPE-efficiency, and $\mu$RD-efficiency.}
\label{fig:rq3-sum}
\end{figure}

\subsection{RQ3: Does the Goodness of Model Consistent with the Resulted Tuning Quality?}

% these best for effieicny might be different for rq1.2 compared with rq1.1

\subsubsection{Method}

To understand \textbf{RQ3}, for each combination of the system and model-based tuner, we select representatives of the best and worst according to a metric. Those are chosen using Scott-Knott ESD test and the average metric value as before. Our goal is to analyze whether the best/worst model, selected by using an accuracy metric, can still lead to the best/worst tuning outcome after the model is used to guide the tuning, assessed by one of the tuning quality metrics. As a result, for sequential model-based tuners, we have 29 systems $\times$ 8 tuners $=232$ cases under an accuracy-quality metric set. Similarly, for the batch model-based tuners, there are 21 large systems $\times$ 8 tuners + 8 small systems $=176$ cases\footnote{Note that for small systems, only \texttt{Brute-force} is needed as the space can be reasonably covered.} per accuracy-quality metric set. Other settings are the same as before.





\input{Tables/RQ2/rq2_smbt}
\input{Tables/RQ2/rq2_bmbt}

\subsubsection{Results}


For sequential model-based tuners, as from Figure~\ref{fig:rq3-sum}, we see a rather low consistency between the model accuracy and the model's tuning performance: there are 16\% and 18\% matched cases (36 and 42 out of 232 cases) on the best representative for MAPE and $\mu$RD, respectively. This is similarly low for the worst representative, exhibiting 16\% and 23\% for MAPE and $\mu$RD (38 and 53 out of 232 cases), respectively. An even lower percentage of matching can be found between model accuracy and tuning efficiency, leading to 26 and 22 out of 232 cases for MAPE and $\mu$RD, respectively, under best representative; 37 and 60 out of 232 cases for MAPE and $\mu$RD, respectively, under worst representative.


The results tend to be more positive for the batch model-based tuners (Figure~\ref{fig:rq3-sum}) in terms of performance, but there are still less than 50\% of the cases show a match on both MAPE and $\mu$RD for the best representative. Similar results can be seen for the scenario of the worst representative: the percentage becomes rather low again when considering efficiency ---16\% and 19\% for MAPE and $\mu$RD (28 and 34 out of 176 cases), respectively, for the best representative. This becomes 17\% and 23\% for the worst representative on MAPE and $\mu$RD (30 and 40 out of 176 cases), respectively.

The difference of matching between sequential and batch model-based tuners is not hard to understand, because the model continues to evolve in the former while it remains fixed for the latter. Therefore, the most/least accurate model could be more indicative and stable of their best/worst performance for batch model-based tuners than that of their sequential counterparts. However, for efficiency, the consistency remains low due to the sparse nature of configuration tuning.   


\begin{figure*}[t!]
\centering
\subfloat{\includegraphics[width=0.6\textwidth]{Figures/rq4-legend.png}}
\vspace{-0.8cm}
\end{figure*}
\begin{figure*}[t!]
\subfloat[sequential model-based tuners]{\includestandalone[width=0.49\textwidth]{Figures/rq4-summary-1}}
~\hfill
\subfloat[batch model-based tuners]{\includestandalone[width=0.49\textwidth]{Figures/rq4-summary-2}}

\caption{Counting the number of cases on the nature/strength for the correlation between accuracy and tuning quality with 30 repeats. The abbreviations are the same as Figure~\ref{fig:rq3-sum}.}
\label{fig:rq4-sum}
\end{figure*}


%\input{Tables/RQ3/rq3_SMBO_perf}
%\input{Tables/RQ3/rq3_SMBO_eff}
%\input{Tables/RQ3/rq3_MFO_perf}
%\input{Tables/RQ3/rq3_MFO_eff}

Tables~\ref{tb:rq3.1} and~\ref{tb:rq3.2} and illustrate the detailed results. We see that, when using certain tuners, it is more likely to have a good consistency between model accuracy and tuning quality of the model than others, e.g., \texttt{OtterTune}, \texttt{ParamILS} and \texttt{ConEx}. The reason behind this can be dependent on how well the tuner balances exploitation and exploration by leveraging the model (see Section~\ref{sec:pair}). Interestingly, we observed that even for \texttt{Brute-force}, there is still a considerable number of mismatched cases. This is because while the overall accuracy might be high, the best-predicted configuration might still be rather erroneous, which prevents it from being effective in guiding the tuning. We will further examine how accurate is enough in \textbf{RQ5}. It is also clear that certain systems lead to more matched cases depending on the tuner type, e.g., \textsc{MongoDB} for sequential and \textsc{MariaDB} for batch model-based tuners. This is due to the tuning landscape of the systems: if the landscape emulated by the model happens to be well-described by the accuracy, then its better or worse is more likely to be consistent with the best/worst tuning quality.

%Overall, we found

\begin{tcbitemize}[%
    raster columns=1, 
    raster rows=1
    ]
  \tcbitem[myhbox={}{Finding \thefindingcount}]  \textit{The sequential model-based tuners lead to generally inconsistent best/worst match between the accuracy and tuning quality of the model (matching in less than 20\% of the cases). The batch model-based tuners, in contrast, have similar results for efficiency but are likely to be more consistent for performance. However, the matching cases are merely up to 45\%.}
\end{tcbitemize}
\addtocounter{findingcount}{1}





==> results-RQ4-5.tex <==
\input{Tables/RQ3/rq3_smbt_perf}
\input{Tables/RQ3/rq3_smbt_eff}
\input{Tables/RQ3/rq3_bmbt_perf}
\input{Tables/RQ3/rq3_bmbt_eff}

\subsection{RQ4: How Do the Model Accuracy and Tuning Quality Correlated?}

\subsubsection{Methods}

For \textbf{RQ4}, our goal is to study the detailed correlation between the changes in accuracy and that of the tuning quality affected by the models. Therefore, we leverage Spearman's rank correlation and the interpretation mentioned in Section~\ref{sec:sta} to analyze the trend therein. We also used statistical tests to verify whether the correlation is statistically significant. Again, there are 232 and 176 cases to investigate for sequential and batch model-based tuners, respectively. Other settings are identical to those of \textbf{RQ3}. Note that to maintain consistency in the correlation analysis, we convert the systems wherein the performance should be maximized by using the additive inverse of the performance value instead. Therefore, for all systems, a negative correlation means the tuning quality becomes worse when the accuracy improves, and vice versa.





\subsubsection{Results}


As from the Figure~\ref{fig:rq4-sum}a, we observe that a negligible correlation between any accuracy and tuning quality has been prevalent for sequential model-based tuners, ranging from 35\% for $\mu$RD-performance to 58\% for $\mu$RD-efficiency. There are also a considerable amount of cases with weak correlations (from 31\% to 47\% cases). This means that, together for between 82\% and 97\% of the cases, the accuracy is unlikely to significantly influence the tuning quality. It is interesting to see that there is a small but noticeable proportion of negative correlation (weak or moderate)---the worse accuracy actually leads to better configuration tuning by a model. This, albeit counter-intuitive, is indeed possible due to the complex change in the structure of the configuration landscape, as we will discuss in Section~\ref{sec:discussion}.

We see similar results between accuracy and tuning efficiency for batch model-based tuners but negative correlations are less likely, as shown in Figure~\ref{fig:rq4-sum}b. When examining the accuracy and performance, batch model-based tuners are more commonly to exhibit positive correlations than their sequential counterparts, i.e., 32\% and 40\% cases respectively for MAPE and $\mu$RD wherein the correlation is positively moderate or above. This matches with the observations of \textbf{RQ3}, where the models provide more inductive and stable guidance for batch model-based tuners. Yet, only up to 9\% cases of the correlations are strong and positive as implied in the general belief.

==> results-old.tex <==
\section{Results and Analysis}\label{sec:results}

%with RQ1, we need to say how difficult is it to directly compare sequential and batch, and say they can be compared via model free indrectly

\subsection{RQ1: The improvement brought by changing the model}

\input{Figures/rq1.2_sum}
\input{Tables/RQ4/SMBO}
\input{Tables/RQ4/MFO}


\input{Tables/RQ5/SMBO}
\input{Figures/rq1.1_res}
% \input{Tables/RQ5/SMBO_eff}
% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.75 \columnwidth]{Figures/pie_charts.pdf}
% 	\caption{The count on the pairwise comparison results between original SMBO and the best SMBO with model replaced. There are overall 192 cases (24 systems $\times$ 8 types of SMBO).}

% 	\label{fig:rq1_pie}
% \end{figure}

\subsubsection{Methods}

To answer RQ1.1, we need to compare the overall optimization. For SMBO, we compare all SMBO and MFO on real benchmark using the same budget. For each SMBO, we select its best performing model as the model representation, and then choose the best performing SMBO among all SMBO as the representative of SMBO. Similarly, for MFO bench to be compared, we use the corresponding budget to ensure they are in the same condition and select the best performing MFO as the representative. Subsequently, for BMBO, we use the best BMBO with the best performing pre-trained model to compare with the MFO bench with the same training budget. 

Regarding RQ1.2, we focus on improving performance and efficiency by substituting the surrogate model in the original SMBO. In order to show the influence of model, we merely modify the surrogate model of the original SMBO method and utilize the approach mentioned in Section~\ref{sec:3.2.1} to generate predictions and uncertainties. 

To enhance result reliability, for both RQ1.1 and RQ1.2, we conducted 30 random repetitions of the experiments and applied Mann-Whitney U-Test mentioned in Section~\ref{sec:3.3.2} to compare the results. Then we use Equation~\ref{eq:Impr.} to calculate the $Impr.$ of the results difference of initial SMBO and SMBO with model replaced.

\subsubsection{Results} 
\ 

\textbf{1) RQ1.1 Reuslts}

Overall, as seen in Table~\ref{fig:left_plot}, when SMBO utilizes its best performing model, there is a significant improvement in both performance and efficiency. Note that if the comparison between the two is not significant, we consider the result as a tie. Focusing on performance, there is a notable positive improvement in 62.50\% (15 out of 24) cases which ranges from 0.10\% to 169.00\% and a significant negative change in 12.50\% (3 out of 24) which ranges from -0.42\% to -0.03\%. Regarding efficiency, there is a significant improvement in 75.00\% (18 out of 24) cases, with the highest improvement reaching up to 50 times in \texttt{SMAC} with \texttt{GP} and only 8.33\% (2 out of 24) cases show significant negative change. On the contrary, In Table~\ref{fig:right_plot}, BMBO performs worse than MFO bench in 95.83\% (23 out of 24)  cases which span from -200.00\% to -0.31\%, while there is a only 4.16\% (1 out of 24) case in which BMBO loses on efficiency. 

\textbf{2) RQ1.2 Reuslts}

From a holistic perspective, it can be seen from Figure~\ref{fig:RQ1_sum} that 81.67\% (156 out of 192) of the cases can make progress in performance and 81.15\% (155 out of 192) of the cases can be improved in efficiency by substitute the surrogate model, within which 48.69\% (93 out of 192) and 36.65\% (70 out of 192) show statistically significant improvement. Specifically, Table~\ref{tb:rq5_perf} shows the detailed results on differenct systems and SMBO that the performance improvement can reach up to 286.62\% by replacing \texttt{OtterTune}'s \texttt{GP} model with \texttt{HINNPerf} in \textsc{KANZI}, and the efficiency improvement can reach up to 699.63\% by modifying \texttt{OtterTune}'s GP model to \texttt{DaL} in \textsc{ExaStencils}. 


\subsubsection{Analysis}
\ 

\textbf{1) RQ1.1 Analysis}

SMBO with model replaced generally outperforms MFO bench, indicating that utilizing SMBO and appropriately replacing models leads to better performance than MFO. On the other hand, there is no universal paradigm for different systems, models, and SMBO. However, for BMBO, using the surrogate model to replace the real space will bring negative effect on performance and most of the results of using the surrogate model or not in efficiency do not show significant differences. This may because some certain BMBO  happen to find genuinely excellent configurations even though the model's predictions are not accurate. Because of this, The excessive volatility results in a lack of significance in the statistical tests.
% Comparing the models of SMBO methods in terms of performance and efficiency, it is observed that the models in the best performing SMBO tend to be more accurate overall, while models for efficiency are relatively less precise. This aligns with the conclusion from RQ2, where the positive correlation of model accuracy with performance is more pronounced.

\textbf{2) RQ1.2 Analysis}


As an overview, the consistent excellence of SMBO with model replaced is indeed thrilling to observe in over 80\% scenarios.  Therefore, RQ1.1 yields a new conclusion for us: it is mostly feasible to improve performance or efficiency by altering the model. From Table~\ref{tb:rq5_perf}, We observe that almost in every system or SMBO, there are instances where replacing the model leads to improvements in efficiency or performance, which inspires us to achieve better results in a particular system by altering the surrogate model.

\begin{quotebox}
\noindent
\textit{\textbf{Answer to RQ1.1}: SMBO with model replaced wins MFO bench in 83.33\% (62.50\% significant)/83.33\% (75\% significant) cases for performance and efficiency and BMBO wins in 0.00\%/75.00\% (20.83\% significant) for performance and efficiency.}

\noindent

\textit{\textbf{Answer to RQ1.2}: In SMBO, 81.67\%/81.15\% of the cases can be improved in performance/efficiency by substituting the surrogate model, from which 48.69\%/36.65\% show statistically significant improvement.} 
\end{quotebox}


\subsection{RQ2: The match of performance/efficiency and model accuracy}

% \begin{table*}[t!]
%   \centering
%   \caption{The best and worst results of PERF. and MAPE in MFO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ1/rq1_perf_MAPE_free.pdf}
  
%   \label{fig:rq1_perf_MAPE_free}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The best and worst results of EFF. and µRD in SMBO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ1/rq1_eff_rank_model.pdf}
  
%   \label{fig:rq1_eff_rank_model}
% \end{table*}



\input{Tables/RQ2/rq2_SMBO_Perf}
\input{Tables/RQ2/rq2_SMBO_Eff}
\input{Tables/RQ2/rq2_MFO_Perf}
\input{Tables/RQ2/rq2_MFO_Eff}
% \input{Figures/RQ2/rq2_result}
\subsubsection{Methods}


 To address RQ2.1 and RQ2.2, we need to rank the performance of optimization and the accuracy of the model within the same optimization method and system. We conducted 30 random experiments for each optimization method, evaluating the results obtained by various optimization methods and the accuracy of the model. In order to compare the 30 random results, we Firstly use Scott-Knott Effect Size Difference explained in Section~\ref{sec:3.3.2} to choose the best outcome group and select the average best if there are more than one member in the best group. 

In the case of SMBO, since the model is trained gradually and multiple models need to be assessed, we recorde the state of the model every ten epochs and used the average accuracy of all recorded models throughout the process for ranking. In total, We analyzed the results of 8 SMBO methods on 24 systems, totaling 192 cases, and 9 MFO methods on 24 systems, totaling 136 cases (small scale system only uses E\_search). For each case, we compare the best and worst performing models in terms of the model of best and worst performance/efficiency with  in accuracy (MAPE/µRD). The results are as follows.

\subsubsection{Results}  
\ 

\textbf{1) RQ2.1 Reuslts}

% \input{Tables/RQ2/RQ2_MFO_old}
% \input{Tables/RQ1/RQ1_SMBO}
\input{Figures/new_rq2_sum}



\textbf{SMBO} Findings: As an overview, the results presented in Figure~\ref{fig:RQ2_sum} indicate that, in terms of MAPE to performance, there is a match in 19.27\% (37 out of 192) of cases between the best MAPE and the best performance, and 18.23\% (35 out of 192) demonstrating a match between the worst accuracy and the worst performance, resulting in an overall success rate of 18.75\% (72 out of 384) matches. Shifting the focus to the alternative µRD to performance, we observe a match in 21.35\% (41 out of 192) of cases between the best accuracy and the best performance, and 25.52\% (49 out of 192) of cases between the worst accuracy and the worst performance, totaling 23.44\% (90 out of 384) successful matches.

\textbf{BMBO} findings: In terms of MAPE to performance, there is a successful match in 46.32\% (63 out of 136) of cases between the best MAPE and the best performance, and 32.35\% (44 out of 136) of cases between the worst accuracy and the worst performance, totaling 39.34\% (107 out of 272) successful matches. For metric µRD emphasizing accuracy ranking, in µRD to performance, there is a match in 42.65\% (58 out of 136) of cases between the best accuracy and the best performance, and 47.05\% (64 out of 136) of cases between the worst accuracy and the worst performance, totaling 41.18\% (112 out of 272) successful matches.

\textbf{2) RQ2.2 Reuslts}


\textbf{SMBO} Findings:  The analysis considering MAPE to efficiency shows a match in 13.54\% (26 out of 192) of cases between the best MAPE and the best efficiency, and 17.18\% (33 out of 192) demonstrating a match between the worst accuracy and the worst efficiency, resulting in an overall success rate of 15.36\% (59 out of 384) matches. Shifting attention to µRD to efficiency, we observe a match in 9.90\% (19 out of 192) of cases between the best accuracy and the best efficiency, and 24.48\% (47 out of 192) of cases between the worst accuracy and the worst efficiency, totaling 17.19\% (66 out of 384) successful matches.

\textbf{BMBO} Findings: As extracted from Table \ref{tb:rq2_MFO_eff}, the assessment of MAPE to efficiency reveals a successful match in 16.91\% (23 out of 136) of cases between the best MAPE and the best efficiency, with 27.21\% (37 out of 136) demonstrating a match between the worst accuracy and the worst efficiency, resulting in an overall success rate of 22.06\% (60 out of 272) matches. For µRD to efficiency, we find a match in 20.59\% (28 out of 136) of cases between the best accuracy and the best efficiency, and 36.03\% (49 out of 136) of cases between the worst accuracy and the worst efficiency, totaling 28.31\% (77 out of 272) successful matches.


\subsubsection{Analysis}

For performance, the final matching results for both BMBO and SMBO do not exceed 50\% which indicates that the model's accuracy is not consistently aligned with performance, as the best and worst performing models do not necessarily have the best or worst accuracy results in over 50\% of cases. When comparing BMBO and SMBO methods, the matching degree for BMBO is approximately twice that of SMBO (MAPE is 2.04 times, and µRD is 2.05 times). This aligns with our intuition, as in BMBO, the model directly guides the search and evaluates the search results, while in SMBO, the model needs to be progressively trained and predict uncertainties, which may result in weaker performance compared to BMBO.

Regarding efficiency, the final matching results for both methods are all weaker than performance, In other words , the model is even more mismatched with efficiency. The matching degree for the SMBO is less than 20\%, suggesting that in SMBO, the relationship between model accuracy and efficiency is very weak, only slightly higher than the 10\% achieved by completely random matching, falling short of 10\%.

% Comparing µRD and MAPE, we observe that in all situations, the match of µRD is slightly greater than MAPE. This suggests that µRD may be a better choice for characterizing model accuracy in both BMBO and SMBO.

\begin{quotebox}
\noindent
\textit{\textbf{Answer to RQ2.1}: In SMBO, there is a match in 18.75\%/23.34\% of cases between model accuracy (MAPE/µRD) and the best and worst performance, and in BMBO, there is a match in 39.34\%/41.18\% of cases between model accuracy (MAPE/µRD) and the best and worst performance.} 

\noindent
\textit{\textbf{Answer to RQ2.2}: In SMBO, there is a match in 15.36\%/17.19\% of cases between model accuracy (MAPE/µRD) and the best and worst efficiency, and in BMBO, there is a match in 22.06\%/28.31\% of cases between model accuracy (MAPE/µRD) and the best and worst efficiency.}
\end{quotebox}


% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of PERF. and MAPE in MFO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_perf_MAPE_free.pdf}
  
%   \label{fig:rq2_perf_MAPE_free}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of PERF. and µRD in MFO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_perf_rank_free.pdf}
  
%   \label{fig:rq2_perf_rank_free}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of PERF. and MAPE in SMBO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_perf_MAPE_model.pdf}
  
%   \label{fig:rq2_perf_MAPE_model}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of PERF. and µRD in SMBO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_perf_rank_model.pdf}
  
%   \label{fig:rq2_perf_rank_model}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of EFF. and MAPE in MFO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_eff_MAPE_free.pdf}
  
%   \label{fig:rq2_eff_MAPE_free}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of EFF. and µRD in MFO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_eff_rank_free.pdf}
  
%   \label{fig:rq2_eff_rank_free}
% \end{table*}S

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of EFF. and MAPE in SMBO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_eff_MAPE_model.pdf}
  
%   \label{fig:rq2_eff_MAPE_model}
% \end{table*}

% \begin{table*}[t!]
%   \centering
%   \caption{The Spearman’s Rank Correlation Test results of EFF. and MAPE in SMBO}
%   \includegraphics[width=0.9\linewidth]{Figures/RQ2/rq2_eff_rank_model.pdf}
  
%   \label{fig:rq2_eff_rank_model}
% \end{table*}

\input{Tables/RQ3/rq3_SMBO_perf}
\input{Tables/RQ3/rq3_SMBO_eff}
\input{Tables/RQ3/rq3_MFO_perf}
\input{Tables/RQ3/rq3_MFO_eff}

\subsection{RQ3: The correlation of performance/efficiency and model accuracy}

\subsubsection{Methods}

To gain a deeper understanding of the role of the model accuracy, a thorough analysis of the results is required. In RQ2, we analyzed the best performing model and the best accuracy model for each system and optimization. Nevertheless, in this RQ, we directly conducted a Spearman's Rank Correlation Test in Section \ref{sec:3.3.2} on the results to assess whether a monotonic relationship exists between the target variable model accuracy and optimization performance. The same as RQ2, we analyze the results of 8 SMBO methods on 24 systems, totaling 192 cases, and 9 BMBO methods on 24 systems, totaling 136 cases. For each case, we perform a Spearman's Rank Correlation Test on the model accuracy (MAPE/µRD) corresponding to performance/efficiency.

\subsubsection{Results}  
\ 

\textbf{1) RQ3.1 performance results}

\textbf{SMBO Findings}: 
As shown in Figure~\ref{fig:rq3_result}, an overall observation reveals that 45.83\% (88 out of 192) of cases exhibit a significant positive correlation, while 13.54\% (26 out of 192) of cases display a significant negative correlation, and 40.63\% (78 out of 192)  of the cases show negligible effect regarding the correlation between MAPE and performance. In Table~\ref{tb:rq3_SMBO_perf}, from the perspective of individual systems, the highest occurrence of a significant positive correlation is found in \textsc{7z}, with 100\% (8 out of 8), while systems like \textsc{KANZI} exhibit a significant negative relationship in 50\% (4 out of 8) of cases. Concerning individual SMBO, those with a strong positive correlation, such as \texttt{SMAC}, reach 79.16\% (19 out of 24), indicating a significant positive relationship between model accuracy and performance. Conversely, those with weaker relationships, like \texttt{ATconf}, show a significant positive correlation only in 20.83\% (5 out of 24) of cases. The highest correlation coefficient is 0.74 in using \texttt{SMAC} in \textsc{LLVM} and the lowest is -0.53 in applying \texttt{ATconf} for \textsc{Brotli}.

For µRD to performance, the overall observation shows that 61.97\% (119 out of 192) of cases exhibit a significant positive correlation between µRD and performance, with 5.24\% (13 out of 248) of cases displaying a significant negative correlation and 31.25\% (60 out of 192) showing no significant effect. On an individual system level, \textsc{MongoDB} stands out with 100\% (8 out of 8) of cases displaying a significant positive correlation, while systems like \textsc{noc-CM-log} exhibit a significant negative relationship in 37.5\% (3 out of 8) of cases. Among individual SMBO, those with a strong positive correlation, such as \texttt{SMAC}, reach 95.83\% (23 out of 24) of cases, indicating a significant positive relationship between model accuracy and performance. Conversely, those with weaker relationships, like \texttt{ATconf}, solely display a significant positive correlation in 25.00\% (6 out of 24) of cases. The correlation coefficient reaches its peak at 0.71 when utilizing \texttt{SMAC} in \textsc{LLVM}, while the lowest value, -0.36, is observed when applying \texttt{BOCA} in the case of \textsc{MariaDB}.

\textbf{BMBO Findings}: 
For BMBO to performance, the correlation between MAPE and performance indicates an overall significant positive impact in 86.03\% (117 out of 136) of cases, with 13.97\% (19 out of 136) of cases showing negligible impact. From the perspective of individual systems, 47.62\% (10 out of 21) of cases exhibit a consistently significant positive relationship across all BMBO methods, while there are instances, such as system \textsc{jump3r} where 75\% (6 out of 8) of cases show no significant improvement. Considering individual BMBO methods, strong correlations are observed, such as \texttt{GA}, where in 100.00\% (16 out of 16) of cases, model accuracy has a significant positive relationship with performance. Conversely, weaker relationships are observed, as in the case of \texttt{BestConfig}, where 57.14\% (10 out of 16) of cases exhibit a significant positive relationship between model accuracy and performance. The correlation coefficient ranges from -0.06 of using \texttt{BestConfig} in \textsc{SaC} to 0.79 of using \texttt{SWAY} in \textsc{7z}.

For another metric, µRD, the overall trend of correlation with performance is similar to MAPE, with 91.91\% (125 out of 136) exhibiting a significant positive impact and 8.09\% (11 out of 136) of cases showing negligible impact. From the perspective of individual systems, 52.38\% (11 out of 21) of cases consistently show a significant positive relationship across all BMBO, while there are cases, such as \textsc{PostgreSQL} where 37.50\% (3 out of 8) of cases show no significant relationship. On an individual BMBO method basis, strong correlations are observed in \texttt{ConEx}, where in 100.00\% (16 out of 16) of cases, model accuracy has a significant positive relationship with performance. Conversely, weaker relationships are observed, as in the case of \texttt{BestConfig}, where 57.14\% (10 out of 16) of cases exhibit a significant positive relationship between model accuracy and performance. The correlation coefficient varies between -0.10, observed when employing \texttt{R\_search} in \textsc{PostgreSQL}, and 0.80, obtained when utilizing \texttt{GGA} in \textsc{JavaGC}.

% \input{Tables/RQ2/RQ2_SMBO}
\input{Figures/RQ3/rq3_result}
% \input{Tables/RQ2/RQ2_SMBO}

\textbf{2) RQ3.2 efficiency results}



\textbf{SMBO Findings}: 
Regarding the correlation between MAPE and efficiency in Table~\ref{tb:rq3_SMBO_eff}, an overall observation reveals that 28.65\% (55 out of 192) of cases exhibit a significant positive correlation, while 26.04\% (50 out of 192) of cases display a significant negative correlation, and 45.31\% (87 out of 192) of cases show no significant effect. Concerning individual SMBO, those with a strong positive correlation, such as \texttt{FLASH}, reach 75.00\% (18 out of 24), indicating a significant positive relationship between model accuracy and performance. Conversely, those with strong negative relationships, like \texttt{ROBOTune}, show a significant negative correlation in 66.67\% (16 out of 24) of cases. The correlation coefficient varies from -0.69 in using \texttt{ROBOTune} in \textsc{noc-CM-log} to 0.49 in ultilizing \texttt{SMAC} in \textsc{ExaStencils}.

Considering µRD to efficiency, the overall observation shows that 29.69\% (57 out of 192) of cases exhibit a significant positive correlation between µRD and performance, with 16.15\% (31 out of 192) of cases displaying a significant negative correlation and 54.17\% (104 out of 192) revealing no significant effect. Among single SMBO, those with a strong positive correlation, still \texttt{FLASH}, reach 66.67\% (16 out of 24), indicating a significant positive relationship between model accuracy and performance. Conversely, those with weaker relationships, like \texttt{SMAC}, show a significant negative correlation in 29.17\% (7 out of 24) of cases. The correlation coefficient covers a range from -0.58 in using \texttt{ROBOTune} in \textsc{noc-CM-log} to 0.58 in ultilizing \texttt{SMAC} in \textsc{MongoDB}.

\textbf{BMBO Findings}: 
As shown in Table~\ref{tb:rq3_MFO_eff}, for BMBO, the correlation between MAPE and efficiency indicates an overall significant positive impact in 45.59\% (62 out of 136) of cases, with 4.41\% (6 out of 136) of cases exhibiting a significant negative impact and 50.00\% (68 out of 136) of cases showing negligible impact. Considering individual BMBO, strong correlations are observed, such as \texttt{R\_Search}, where in 87.50\% (14 out of 16) of cases, model accuracy has a significant positive relationship with performance. Conversely, weaker relationships are observed, as in the case of \texttt{Irace}, where 6.25\% (0 out of 16) exhibit a significant positive relationship between MAPE and performance. The correlation coefficient goes from -0.28 in using \texttt{E\_search} in \textsc{Brotli} to 0.76 in ultilizing \texttt{R\_search} in \textsc{HIPAcc}.

For another metric, µRD, and its correlation with performance, the overall trend mirrors that of MAPE. Out of 136 instances, 51.47\% (70 cases) display a significant positive impact, 4.41\% (6 cases) show a negative impact, and 44.12\% (60 cases) show no significant impact. On an individual basis for each BMBO method, robust correlations are evident in \texttt{R\_Search} demonstrating a strong relationship with model accuracy having a significant positive impact in 100.00\% (16 out of 16) of cases. Conversely, weaker relationships are observed, such as in the case of \texttt{Irace}, where 0.00\% (0 out of 16) exhibit a significant positive or negative relationship between µRD and performance. The correlation coefficient extends from -0.20 in using \texttt{BestConfig} in \textsc{storm} to 0.75 in ultilizing \texttt{R\_search} in \textsc{7z}.

\subsubsection{Analysis}
The final correlation results indicate that, for SMBO ,there is a positive effect on performance in approximately 50\% of cases, with negative or unclear effects in the remaining cases. Therefore, improving the accuracy of the performance model may not necessarily change the results. Additionally, for Efficiency, solely 28.65\% and 29.69\% show positive effects, and even in MAPE, the significantly negative effects almost catch the positive ones. This is an interesting finding, suggesting that in SMBO, the accuracy of the model may have a negative impact on efficiency.


For BMBO, there is a high likelihood (over 85\%) of a significant positive relationship between Performance and accuracy. Additionally, there is still a significant positive relationship (over 40\%) between efficiency and accuracy, with only less than 5\% exhibiting a negative relationship. Additionally, \texttt{R\_search} and \texttt{E\_search}, the classic BMBO still shows significantly stronger correlation than other BMBO in efficiency. This may because they directly sample and search randomly, other BMBO methods have their own search rules and are not entirely model-driven, resulting in lower correlation effect compared to the search BMBO. When looking at individual methods within BMBO, \texttt{BestConfig} and \texttt{Irace} effect is lower than in other BMBO, possibly due to they use their own stronger influence rule to search and being less sensitive to model accuracy.


% Moreover, regarding the metrics µRD and MAPE, the negative effects observed in MAPE are almost twice those in µRD. This indicates that if one aims to improve search results by enhancing model accuracy, it is advisable to focus on µRD, which involves relative ranking accuracy rather than optimizing absolute accuracy.


\begin{quotebox}
\noindent

\textit{\textbf{Answer to RQ3.1}: In SMBO, there is a positive correlation of 45.83\%/61.97\% between performance and model accuracy (MAPE/µRD), in BMBO, there is a positive correlation of 86.03\%/91.91\% between performance and model accuracy (MAPE/µRD).}


\textit{\textbf{Answer to RQ3.2}: In BMBO, there is a positive correlation of 28.65\%/29.69\% between efficiency and model accuracy (MAPE/µRD), in SMBO, there is a positive correlation of 45.59\% and 51.47\% between efficiency and model accuracy (MAPE/µRD).}
\end{quotebox}


\subsection{RQ4: The model accuracy change we need to make}

\input{Figures/test}
\input{Figures/test_rang1}

\input{Figures/test1}
\input{Figures/test_rang2}

\subsubsection{Methods}

To address RQ4, a more nuanced examination is required. Thus, we conduct further analysis on the results, extracting instances where accuracy (MAPE/µRD) change is associated with a significant enhancement in performance/efficiency. For the significance testing, we employed the Mann-Whitney U-test in Section~\ref{sec:3.3.2}. Note that among several pairs demonstrating improvements with model changes, we selected the pair with the least increase or decrease in model accuracy as the desired threshold for accuracy improvement.

% \input{Tables/RQ3_rank}
% \input{Tables/RQ3_MAPE}


\subsubsection{Results}

From the Figure~\ref{fig:RQ4_MAPE} and Figure~\ref{fig:RQ4_rank}, we observe that for all methods in both SMBO and BMBO, a significant improvement in results can be achieved with an increase of approximately 1\% in accuracy when the accuracy is below 10\%. As the accuracy interval increases, progressively more accuracy change is required to achieve a significant enhancement in results. The distribution of data is shown in Figure~\ref{fig:RQ4_MAPE_range} and Figure~\ref{fig:RQ4_rank_range} which give us an overall accuracy description.
\subsubsection{Analysis}

As accuracy increases, the required increment in accuracy for a significant change also grows, aligning with our expectations.
Comparing SMBO and BMBO, overall, SMBO tends to require a smaller change in accuracy to achieve a significant change compared to BMBO. This may be attributed to the sampling and training process in SMBO, where the model plays a more crucial role, leading to a more substantial impact.


\begin{quotebox}
\noindent

\textit{\textbf{Answer to RQ4}: When the accuracy is below 10\%, both BMBO and SMBO require an change of approximately 1\% to achieve a significant change in results, and subsequently, as the accuracy increases, the required accuracy change for a significant change gradually becomes higher.}

\end{quotebox}

% \input{Figures/RQ4/rq4_results}


==> threats_to_validity.tex <==
\section{threats to validity}\label{sec:threats}

This section elaborates on the potential threats to the validity of our study.

\subsection{Internal Threats} Internal threats are the potential biases introduced by the research design or methodology that may impact the accuracy or reliability of the findings:

\begin{itemize}
\item \textbf{Budget:} Tuning budget is highly specific in different scale systems and SMBO as well as MFO. To tackle this, We design and conduct pre-experiments to decide this parameter to ensure all optimization can reach their search end. On the other hand, the Training budget in MFO is determined following the methodology proposed by Li et al. \cite{siegmund2015performance}. Moreover, in order to make the pre-trained model as good as possible, we chose the largest one among multiple budgets generated.
\item \textbf{Initial size:} To ensure fairness and consistency, we have opted for an initial size of 20, which is widely used and considered relatively larger. While this size may not be ideal for extensive space systems, our self-adaptive tuning budget can effectively alleviate this concern by guiding the optimization process toward its intended destination.
\item \textbf{Optimizer setting:} We use 8 MFO and 8 SMBO optimization methods, of which the hyperparameters are set as close as possible to the original settings except for the initial size which should be consistent among all SMBO and overall budget being regular for comparison fairness. 

\end{itemize}

\subsection{Construct Threats} Threats to construct validity may lie in the following aspects:

\begin{itemize}
\item \textbf{Metric:} Ten models are included in the experiments and accuracy of them need to be measured properly. We use MAPE for the purpose of measuring the absolute accuracy of the models and comparing among various systems \cite{MAPE1}. Considering the shortcoming of MAPE, µRD is used with the aim of measuring rank difference of model with the real space, and we make some minor changes to address the issue of inconsistent sample size of varied systems \cite{flash}.
\item \textbf{Statistics:} In every experiment, the results of SMBO and MFO have a certain randomness. To eliminate this randomness to some extent, we conducted 30 random experiments. For multiple results of the experiments, we use Mann-Whitney U-Test and Scott-Knott ESD Test to conduct pairwise comparison and group comparison to the results which makes results convincing.

\item \textbf{Noises:} The measured system performance might be inferred by low-level perturbation, e.g., OS activities and hardware
instability. This can be partially tackled by repeated measurements and the above stiasitical test. However, we admit that completely removing those noises is impossible.  

\end{itemize}

\subsection{External Threats} External validity refers to limitations in the generalizability of the findings to other populations, such as the selection of subject systems and training samples:

\begin{itemize}
    \item \textbf{Software systems:} In this paper, we have included 24 diverse software configuration systems from previously conducted research. These systems span across various fields and possess varying scales and optimization objectives. While we acknowledge that this collection of software systems is not exhaustive, we aim to consider an even more comprehensive range of systems in the future.
    \item \textbf{Optimization methods:} In this study, a comprehensive analysis is conducted using 8 MFO and 8 SMBO methods. Some of the methods are regarded as the state-of-the-art techniques and the others are classical optimizer. Therefore, we believe that the results of empirical research are representative, but we can incorporate more methodology in the future to extend our study.
    \item \textbf{Models:} We utilize ten surrogate models for optimization purposes. Given that Deep Neural Network (DNN) models demand considerable time and resources for parameter tuning and optimization, we refrain from performing parameter tuning on intricate models, which could potentially result in inferior model performance. Our objective, however, is to investigate the influence of model accuracy on the final results and we regard that this approach do not hinder the validity of our conclusions.
    \item \textbf{Number of objectives:} Our work only select one goal of each system for optimization, hence the results may not be very suitable for multi-objective cases. We look forward to expanding this work to obtain more widely applicable conclusions for multi-objective fields.
\end{itemize}

